A Unified Approach for Multi-Scale Synchronous Correlation Search in Big Time Series -- Full Version

The wide deployment of IoT sensors has enabled the collection of very big time series across different domains, from which advanced analytics can be performed to find unknown relationships, most importantly the correlations between them. However, current approaches for correlation search on time series are limited to only a single temporal scale and simple types of relations, and cannot handle noise effectively. This paper presents the integrated SYnchronous COrrelation Search (iSYCOS) framework to find multi-scale correlations in big time series. Specifically, iSYCOS integrates top-down and bottom-up approaches into a single auto-configured framework capable of efficiently extracting complex window-based correlations from big time series using mutual information (MI). Moreover, iSYCOS includes a novel MI-based theory to identify noise in the data, and is used to perform pruning to improve iSYCOS performance. Besides, we design a distributed version of iSYCOS that can scale out in a Spark cluster to handle big time series. Our extensive experimental evaluation on synthetic and real-world datasets shows that iSYCOS can auto-configure on a given dataset to find complex multi-scale correlations. The pruning and optimisations can improve iSYCOS performance up to an order of magnitude, and the distributed iSYCOS can scale out linearly on a computing cluster.

==> applyNoiseTheoryToBU_bk.tex <==
\subsection{Using Noise Theory to Improve SYCOS$_{\text{BU}}$}\label{sec:improveBU} 
In this section, we discuss how to apply the noise theory to prune irrelevant data partitions during two different exploration phases of SYCOS$_{\text{BU}}$: initial solution finding and neighborhood exploration. 
\subsubsection{Initial noise pruning} Recall that SYCOS$_{\text{BU}}$ starts with an initial solution $w_0$, and tries to improve $w_0$ through neighborhood exploration. An initial solution can be initialized in different ways, for example, $w_0$ can start at the beginning or at an arbitrary location in the time series. However, this random initialization can lead the search to an unpromising exploration area. For instance, if the search starts at the valleys in Fig. \ref{fig:mifluctuation}, it will take longer time to reach the top of the hill than if it starts on the slopes. 
To avoid such unpromising "valley-trapped" situations, we apply Theorem \ref{theorem:noise} to assist SYCOS$_{\text{BU}}$ in finding a good starting point. 

SYCOS$_{\text{BU}}$ is at a good starting point if the initial solution $w_0$ has $I_{w_0} \ge \tau$ (the \textit{noise threshold}). To find such a point, we first divide the time series into non-overlapping windows of the minimal size $s_{\min}$, and then hierarchically combine them to form larger, and hopefully better windows. The combination stops when it finds a window $w$ that has $I_w \ge \tau$. 
Fig. \ref{fig:pruning} demonstrates this procedure.


\begin{figure}[!h]
	\vspace{-0.07in}
	\centering
	\begin{tikzpicture}
	\tikzset{
		cross/.pic = {
			\draw[rotate = 45, line width=0.5mm, cap=round] (-#1,0) -- (#1,0);
			\draw[rotate = 45, line width=0.5mm, cap=round] (0,-#1) -- (0, #1);
		}
	}
	\newcommand{\drawlinerror}[5]{
		\draw[#1, line width=0.5mm, cap=round] (axis cs: #2, #3) -- (axis cs: #2+#4,#3);
		\path (axis cs: {#2+#4/2+0.5}, #3) pic[red] {cross=7pt};
		\node[black] at (axis cs: {#2+#4/2+0.5}, #3-2) {\small #5};
	}
	
	\newcommand{\drawline}[5]{
		\draw[#1, line width=0.5mm, cap=round] (axis cs: #2, #3) -- (axis cs: #2+#4,#3);
		\node[black] at (axis cs: {#2+#4/2+0.5}, #3-2) {\small #5};
	}
	
	\begin{axis}[axis line style={draw=none},
	tick style={draw=none},
	ymin = 0, ymax = 50,
	xmin = 0, xmax = 50,
	xticklabels={,,},
	yticklabels={,,}
	]
	
	\draw [black,thick, -latex] (axis cs: 12, 3) -- (axis cs: 50,3) node [right] {};
	\node[black] at (axis cs: 48, 1) {\small $T$};
	
	% \node[black] at (axis cs: 5, 8) {\small Step 1};
	\node[black] at (axis cs: 5, 8) {\small Step 1\hphantom{.0}};
	\drawline {black!30!green}{12}{8}{8}{$W_1$}
	\drawline {black!30!green}{21}{8}{8}{$W_2$}
	
	\node[black] at (axis cs: 5, 15) {\small Step 2\hphantom{.0}};
	\drawline {black!30!green}{12}{15}{16.5}{$W_{12}$}
	
	\node[black] at (axis cs: 5, 23) {\small Step 3.1};
	\drawline {black!30!green}{12}{23}{16.5}{$W_{12}$}
	\drawline {black!30!green}{29.5}{23}{8}{$W_3$}
	
	\node[black] at (axis cs: 5, 30) {\small Step 3.2};
	\drawline {black!30!green}{12}{30}{25}{$W_{123}$}
	
	\node[black] at (axis cs: 5, 37) {\small Step 3.3};
	\drawlinerror {black!30!green}{12}{37}{16.5}{$W_{12}$}
	\drawlinerror {black!30!green}{29.5}{37}{8}{$W_3$}
	
	\node[black] at (axis cs: 5, 44) {\small Step 4\hphantom{.0}};
	\drawline {black!30!green}{29}{44}{8}{$W_3$}
	\drawline {black!30!green}{38}{44}{8}{$W_4$}
	\end{axis}
	\end{tikzpicture}
	\caption{Illustration of hierarchical combination}
\label{fig:pruning}
\vspace{-0.05in}
\end{figure} 

In \textit{Step 1}, initially the search starts with two minimal consecutive and non-overlapping time windows $w_1$, $w_2$, and evaluates their goodness by computing $I_{w_1}$, $I_{w_2}$. In \textit{Step 2}, it combines the \textit{two} windows into a bigger one $w_{12}$, and computes $I_{w_{12}}$. Next, it compares the goodness of the \textit{three} windows, and select the one that has the highest MI. Assuming that $\{I_{w_1}, I_{w_2}\} \le I_{w_{12}} < \tau$, then $w_{12}$ is the one selected among the \textit{three}. Since $I_{w_{12}}$ is still less than $\tau$, it moves to \textit{Step 3.1}, where a next minimal window $w_3$ is evaluated both separately (by computing $I_{w_3}$), and together with $w_{12}$ (by computing $I_{w_{123}}$). 

Assume that $I_{w_3} < \tau$, and that by combining $w_3$ to $w_{12}$, it reduces the MI $I_{w_{12}}$, i.e., $I_{w_{123}} < I_{w_{12}} < \tau$. According to Theorem \ref{lem:noise1}, we can conclude that $w_3$ is noise w.r.t. $w_{12}$. Thus, the combination $w_{123}$ does not lead to a promising result. The next window to be considered is $w_4$. However, $w_{12}$ cannot be combined with $w_4$ without the presence of $w_3$, which we know is noise of $w_{12}$. Thus, the combination $w_{1234}$ should not be formed, and $w_{12}$ should also be eliminated from future consideration (\textit{Step 3.3}). Next, in \textit{Step 4}, $w_3$ is evaluated again in combination with $w_4$, and the procedure is repeated until it can find a window that has MI $> \tau$. Once a good starting point is determined, SYCOS$_{\text{BU}}$ begins its neighborhood exploration as described in Section \ref{sec:bottomup}. 

\textit{Ensuring the completeness of SYCOS$_{\text{BU}}$} When SYCOS$_{\text{BU}}$ stops at a locally optimal solution, it has followed the best path and explored to the deepest level of the current tree. This, however, does not guarantee that is the only path. In fact, as stated in the problem formulation (Eq. \eqref{eq:pbformulation}), we want to find a set of all windows that are above the correlation threshold. Thus, to ensure the completeness of the search, we design SYCOS$_{\text{BU}}$ in a recursive way such that once it stops at the locally optimal solution, it goes back to the previously found starting point and continues exploring other paths to find all potential solutions.   

\subsubsection{Subsequent noise detection}
The noise theory is also useful during the neighborhood exploration process. We explain its applicability in Fig. \ref{fig:searchspacebf}. Assuming that $w$ is the current window, and $w^{l}_{N_1}$, $w^{l}_{N_2}$ are its neighbors when the search moves leftwards. 
In the first exploration, the neighbor $w^{l}_{N_1}$ is considered. Since $w^{l}_{N_1}$ is created by extending the start index of $w$ by an $\delta_1-$step to the left, we have: $w^{l}_{N_1}= w_{\delta_1} \odot w$ where $w_{\delta_1}$ is the extension to be added to $w$. Also assuming that by applying our noise theory to $w$, $w_{\delta_1}$, and $w^{l}_{N_1}$, we conclude that $w_{\delta_1}$ is noise w.r.t. $w$, then it is not promising to explore further the leftwards neighborhoods of $w$. Thus, in the next exploration, SYCOS$_{\text{BU}}$ should omit $w^{l}_{N_2}$, and remove the leftwards direction entirely from its search. 

However, to ensure that the noise theory does not overuse and thus, might remove important data, we use a parameter $p$ to count the number of times the noise theory has been continuously applied successfully in the same exploration direction. Only when $p$ number of times noises have been continuously identified in the considered direction, SYCOS$_{\text{BU}}$ will stop explore that direction. For instance, in the example above, after identifying that $w_{\delta_1}$ is noise w.r.t. $w$, SYCOS$_{\text{BU}}$ does not stop exploring the leftwards direction immediately but does so only if noises have been detected continuously $p$ number of times.    

%\input{bounds}
%Algorithm \ref{alg:improvedSYCOS} reflects on how the noise theory in Section \ref{sec:noisetheory} and MI bound in Section \ref{sec:bound} are applied to SYCOS$_{\text{BU}}$. 
Algorithm \ref{alg:improvedSYCOSBU} reflects on how the noise theory in Section \ref{sec:noisetheory} is applied to SYCOS$_{\text{BU}}$. 
In line $2$, the noise theory is applied to find a good starting point (initial solution) for SYCOS$_{\text{BU}}$. %The MI bound estimation is used to estimate $\delta$ value in line $5$. 
During the neighborhood exploration, the noise theory is applied again to prune the search space (line $6$).
\begin{algorithm}[!h]
	\caption{Improve SYCOS$_{\text{BU}}$ using the noise theory}
	\small
	\begin{algorithmic}[1]
		\Statex{{\bf Input:}} $(X_T,Y_T)$: \text{pair of time series} 
		\Statex{{\bf Params:} $\sigma$: \text{correlation threshold,}}
		\Statex{\hspace{1.23cm}$\tau$: \text{noise threshold,}}
		\Statex{\hspace{1.23cm}$p$: \text{number of times noises have been identified,}}
		\Statex{\hspace{1.23cm}$s_{\max}$: \text{maximum size,}} 
		\Statex{\hspace{1.23cm}$s_{\min}$: \text{minimum size}}  	
		\Statex{{\bf Output:} $\mathit{S}$: \text{set of non-overlapping windows whose MI $ \ge \sigma$}}
		\While{$(X_T,Y_T)$ does not empty}
		\State $w:=w_0$ with $w_0 :=$\textit{InitialNoisePruning}$((X_T,Y_T),\tau)$ \Comment{Apply Theorem \ref{lem:noise1} to find a good initial solution}
		\State Compute $I(w)$ \Comment{Evaluate the goodness of $w$}
		\While {$T_{idle} < T_{maxIdle}$}
		%\State $\delta$ := \textit{EstimateDelta}$(R(w),\sigma)$ \Comment{Apply MI bound to estimate $\delta$}
		\State $N := \textit{Neighbors}(w)$ \Comment{Identify the neighbors of $w$}
		\State $N^{'} := \textit{SubsequentNoiseDetection}(N,\tau,p)$ \Comment{Apply Theorem \ref{lem:noise1} to prune unpromising neighbors in $N$} 
		\State $w_{best}:=$ \textit{BestNeighbor}($N^{'}$)\Comment{Select the best neighbor in $N^{'}$ based on the goodness measure}
		\State $w_h:=$ \textit{random.get(\textbf{$L_h$})} \Comment{Randomly select an element from the history \textbf{$L_h$}}
		\State $w:=$\textit{EvaluateCandidateSolution}$(w,w_h,w_{best})$ \Comment{Follow the steps 13-22 in Algorithm \ref{alg:bottomupsearch} to evaluate the candidate $w_{best}$}
		\EndWhile
		\If{$I_w \ge \sigma$}
		\State Insert $w$ to $S$ 
		\EndIf  
		\State SYCOS$_{\text{BU}}$$(X^{'}_T,Y^{'}_T)$ \Comment{Restart SYCOS$_{\text{BU}}$ on the remaining of $(X_T,Y_T)$}
		\EndWhile
		\State \textbf{return} $S$
	\end{algorithmic}
	\label{alg:improvedSYCOSBU}
\end{algorithm}

==> bottomup.tex <==
\subsection{SYCOS$_{\text{BU}}$: Bottom-Up  Search}\label{sec:bottomup}
%We propose two approaches to search for correlated time windows: bottom-up and top-down. 
In this section, we describe the bottom-up method SYCOS$_{\text{BU}}$ that employs Late Acceptance Hill Climbing algorithm to search for correlated windows. The idea of the bottom-up search approach is to start with small-size windows, and then enlarges the window's size as the search progresses. %In contrast, the top-down approach, SYCOS$_{\text{TD}}$, starts with large-size windows, and reduces the window sizes if the series in large-size windows are not well correlated. 
This implies that SYCOS$_{\text{BU}}$ assumes correlations exist in small-size windows, and thus is more efficient to start with small windows. %Through empirical experiments in Section \ref{sec:experiment}, we show that both assumptions are valid and hold for real case studies, and depending on the case studies, one approach can be superior to another.    

\subsubsection{Late Acceptance Hill Climbing}
Late Acceptance Hill Climbing \cite{burke2017late}, an extension of the classic Hill Climbing (HC) \cite{russell2016artificial}, is an optimization technique attempting to find locally optimal solutions for a given problem through iterative improvement. Given a \textit{target function} $f$ and a current solution $S$ of $f$, LAHC tries to improve $S$ by exploring potential candidates in the nearby neighborhood. 
If a better solution is found (according to the predefined objectives), the current solution $S$ is replaced by this new solution $S_{\text{new}}$, and the process is repeated until no further improvement can be made.   

LAHC differs from the classic HC in its acceptance rule, i.e., it can accept a solution $S_{\text{new}}$ if $S_{\text{new}}$ is better than either the current solution $S$ or a solution $S_{\text{old}}$ found in the history. To do that, LAHC uses a fixed length array $L_h$ to maintain a history of the most recently accepted solutions, and use this $L_h$ array to justify the goodness of a candidate solution. 

One of the challenges of LAHC (or HC in general) is the convergence to \textit{local optima}. A \textit{local optimum} is a situation where the technique converges to a local best solution, but not necessarily the globally optimal one \cite{russell2016artificial}. However, in the following sections, we explain that \textit{local optima} are in fact what we are looking for in SYCOS problem.

\subsubsection{Apply LAHC to SYCOS}
We consider the problem of searching for synchronous correlations, i.e., SYCOS, using LAHC as a \textit{maximization} problem. Specifically, the \textit{target function} of LAHC is a \textit{maximize} function, and our goal is to search for the time windows where their MIs are locally maximal. %Thus, given a pair of time series $(X_T,Y_T)$, and the \textit{target function} $I_w=I(X_w;Y_w)$, the SYCOS problem becomes: 
%%\begin{equation}
%%\begin{split}
%%\text{SYCOS}_{\text{BU}} (X_T,Y_T) &:=\{ w_i \mid I(X_{w_i};Y_{w_i}) \ge \sigma \\&
%%\hspace{-0.5in}\wedge I(X_{w_{i-1}};Y_{w_{i-1}}) \le I(X_{w_i};Y_{w_i}) \\&
%%\hspace{-0.5in}\wedge I(X_{w_{i+1}};Y_{w_{i+1}}) \le I(X_{w_{i}};Y_{w_{i}})
%%\} 
%%\end{split}
%%\label{eq:pbformulation}
%%\end{equation}
%%Eq. \ref{eq:pbformulation} represents a set of all windows $w_i$ whose MIs are locally maximal values that satisfy the correlation threshold.  
%\textit{Why are local optima the solutions of SYCOS$_{\text{BU}}$?}
 %is LAHC a good candidate solution for correlation search?}}
To explain why local optima are in fact the solutions of SYCOS$_{\text{BU}}$, consider Fig. \ref{fig:mifluctuation} that plots the fluctuation of MI values for a given pair of variables. Here, the $y-$axis represents the MI values of the time windows on the $x-$axis. Given the correlation threshold $\sigma$ (red line in Fig. \ref{fig:mifluctuation}), the three windows which correspond to the three maximal points (in red) indicate highly correlated areas (above $\sigma$). %the search will extract three different windows which correspond to three maximal points (in red) which is above $\sigma$
These windows can be found by first identifying the three peak points which represent the locally maximal MI values, and then extending the located points to the surrounding areas to determine the precise window's indices. Such windows are guaranteed to satisfy the correlation condition: $I_w \ge \sigma$. 

\begin{figure}[!h]
	\vspace{-0.12in}
	\centering
	\includegraphics[width=0.35\textwidth]{figures/MIFluctuation2D} %{figures/MI1} {figures/MI2}
	\vspace{-0.1in}
	\caption{Mutual information fluctuation}
	\label{fig:mifluctuation}
	\vspace{-0.1in}
\end{figure}
%Since an LAHC-based method guarantees local optimal solutions, it is an ideal solution for SYCOS. % for general problems, and global optimal solutions for convex problems \textbf{need citation}. %– otherwise it will find only local optima (solutions that cannot be improved by considering a neighboring configuration), which are not necessarily the best possible solution (the global optimum) out of all possible solutions (the search space). Examples of algorithms that solve convex problems by hill-climbing include the simplex algorithm for linear programming and binary search.[1]:253 To attempt overcoming being stuck in local optima, one could use restarts (i.e. repeated local search), or more complex schemes based on iterations (like iterated local search), or on memory (like reactive search optimization and tabu search), or on memory-less stochastic modifications (like simulated annealing).
%The property to guarantee local optimal solutions makes Hill Climbing a perfect candidate to search for temporal correlations in time series. We explain how this property makes the method a perfect candidate for correlation search in the next section. %Other properties such as the simplicity and the ability to provide valid solution at anytime make the algorithm a popular choice amongst other optimization algorithms. 
%\textit{Why finding local optima is a good property for temporal correlation search?} because finding correlations in time series means to maximize the MI within a certain time duration, which implies the local optimal among the entire time series.

%Indeed, finding correlations in time series means to find the time windows that maximize the MI, which implies finding the locally optimal solutions that are above the correlation threshold.
Since an LAHC-based method guarantees local optimal solutions, it is an ideal technique for SYCOS. Moreover, during the search process, an LAHC-based method does not maintain a complete search tree since it looks only at the current state and neighbor states, thus is memory efficient. %This is another advantage of using LAHC-based methods for correlations search. % in big time series. 

\textit{Definition 5.1} \textit{($\delta$-neighbor)} Let $(X_T,Y_T)$ be a pair of time series of length $n$ measured during the time interval $T$, and $w=[t_s,t_e]$ be a time window of $(X_T,Y_T)$. A window $w^{'}=[t_s^{'},t_e^{'}]$ is an \textit{$\delta$-neighbor} of $w$ if $(t_s^{'}=t_s-\delta$ $\vee$ $t_s^{'}=t_s+\delta)$  $\vee$ $(t_e^{'}=t_e-\delta$ $\vee$ $t_e^{'}=t_e+\delta)$, where $\delta$ is a pre-defined moving step such that $1 \le \delta \le n$ $\wedge$ $s_{\min} \le \abs{w^{'}} \le s_{\max}$. 
\\
\textit{Definition 5.2} \textit{($\delta$-neighborhood)} Let $w=[t_s,t_e]$ be a time window of $(X_T,Y_T)$. A \textit{$\delta$-neighborhood} $N$ of $w$, denoted as $N_{\delta}$, is the surrounding area of $w$ formed by all \textit{$\delta$-neighbors} $w^{'}=[t_s^{'},t_e^{'}]$ of $w$. 

\begin{figure}[!h]
	\centering
	\resizebox{.7\linewidth}{!}{
	\begin{tikzpicture}%[scale=0.8]
	\begin{axis}[inner axis line style={black},
	axis lines=center,axis line style={-latex},
	tick style={draw=none},
	ymin = 0, ymax = 15,
	xmin = 0, xmax = 12,
	xscale=1.3,
	xticklabels={,,},
	yticklabels={,,},
	xlabel=$t_s$,
	ylabel=$t_e$,
	xlabel style={
		at={(ticklabel cs:0.95)},
		anchor=west,
	},
	ylabel style={
		at={(ticklabel cs:0.95)},
		anchor=south,
	}
	]
	\coordinate (O) at (axis cs:0,0);
	\coordinate (X) at (axis cs:1,0);
	\coordinate (Y) at (axis cs:0,1);
	\end{axis}  
	\begin{scope}[x={($(X)-(O)$)}, y={($(Y)-(O)$)}, shift={(O)}]
	
	
	\foreach \v in {1,2,...,\cols} {
		\pgfmathsetmacro{\ynew}{(1+(\v-1)*\kcachy)}
		\drawdot{black}{\v}{\ynew}{\rows}{\kcach}; 
	};
	
	\foreach \v in {1,2,...,\rows} {
		\draw [black] (1, {(1+(\v-1)*\kcach)}) -- (\cols, {(1+(\cols-1)*\kcachy)+(\v-1)*\kcach)});
	};
	
	\foreach \v in {3,4,...,7} {
		\pgfmathsetmacro{\Y}{(1+(\v-1)*\kcachy)}
		\pgfmathsetmacro{\ynew}{(\Y+\kcach)}
		\drawdot{blizzardblue}{\v}{\ynew}{5}{\kcach}; 
	};
	
	\foreach \v in {4,5,6} {
		\pgfmathsetmacro{\Y}{(1+(\v-1)*\kcachy)}
		\pgfmathsetmacro{\ynew}{(\Y+2*\kcach)}
		\drawdot{blue-violet}{\v}{\ynew}{3}{\kcach}; 
	};
	\node [circle,draw=black, fill=blue, scale=0.6] (center) at (5, {(1+4*\kcachy+3*\kcach)}) {};
	
	\draw [black, dashed] (0,1) -- (1,1);
	\draw [black, dashed] (0,{(1+(\rows-1)*\kcach)}) -- (1,{(1+(\rows-1)*\kcach)});
	\draw [black, dashed] (1,0) -- (1,1);
	\draw [black, dashed] (0,{((1+(\cols-1)*\kcachy)+(\rows-1)*\kcach)}) -- (\cols,{((1+(\cols-1)*\kcachy)+(\rows-1)*\kcach)});
	\draw [black, dashed] (\cols,0) -- (\cols,{((1+(\cols-1)*\kcachy)});
	
	\node [red] at (-0.6,1) {\small $t_{e_{11}}$};
	\node [red] at (-0.6,{(1+(\rows-1)*\kcach)}) {\small $t_{e_{1l}}$};
	
	\node [red] at (1,-0.6) {\small $t_{s_{1}}$};
	\node [blue] at (\cols,-0.6) {\small $t_{s_{m}}$};
	
	\node [blue] at (\cols+1,{((1+(\cols-1)*\kcachy)}) {\small $t_{e_{m1}}$};
	\node [blue] at (\cols+1,{((1+(\cols-1)*\kcachy)+(\rows-1)*\kcach)}) {\small $t_{e_{ml}}$};
	
	\node [blue] (iw) at (-0.9,7) {$I_w$};
	\draw [-latex, dashed, blue] (iw) -- (center);
	
	\node [blue] at (5.4, {(1+4*\kcachy+1*\kcach)+0.6}) {\tiny $W^b_{N2}$};
	\node [blue] at (5.4, {(1+4*\kcachy+2*\kcach)+0.6}) {\tiny $W^b_{N1}$};
	\node [blue] at (5.4, {(1+4*\kcachy+4*\kcach)+0.6}) {\tiny $W^t_{N1}$};
	\node [blue] at (5.4, {(1+4*\kcachy+5*\kcach)+0.6}) {\tiny $W^t_{N2}$};
	
	\node [blue] at (5.2, {(1+4*\kcachy+3*\kcach)+0.6}) {\tiny $W$};
	
	\node [blue] at (3.4, {(1+3*\kcachy+3*\kcach)-0.7}) {\tiny $W^l_{N2}$};
	\node [blue] at (4.4, {(1+4*\kcachy+3*\kcach)-0.7}) {\tiny $W^l_{N1}$};
	\node [blue] at (6.4, {(1+6*\kcachy+3*\kcach)-0.7}) {\tiny $W^r_{N1}$};
	\node [blue] at (7.4, {(1+7*\kcachy+3*\kcach)-0.7}) {\tiny $W^r_{N2}$};

	\end{scope}
	\end{tikzpicture}
}
\vspace{-0.1in}
\caption{Search space for SYCOS$_{\text{BU}}$}
\label{fig:searchspacebf}
\end{figure}

%%\begin{figure}[!h]
%%	\centering
%%	\includegraphics[width=0.35\textwidth]{figures/bruteforce_new}
%%	\vspace{-0.1in}
%%	\caption{Search space for SYCOS$_{\text{BU}}$ \textbf{to fix the missing lines}}
%%	\label{fig:searchspacebf}
%%\end{figure}

We illustrate the \textit{neighborhood} concept in Fig. \ref{fig:searchspacebf}. % that represents the search space of SYCOS$_{\text{BU}}$. 
Here, each point in the grid represents a time window with the x-axis represents the start time, and the y-axis represents the end time. Consider the window $w$ in blue. The nearest $\delta-$neighborhood of $w$, called the $1-$neighborhood $N_1$, is the area formed by the \textit{eight} windows in light purple color surrounding $w$. Each window in this neighborhood differs from $w$ by \textit{one} $\delta$ step, either by its start index, or its end index, or both. Going further from $w$, the next neighborhood of $w$, called the $2-$neighborhood $N_2$, is the $16$ windows in light blue color. Each $\delta-$\textit{neighborhood} will form an area where LAHC will iteratively look for potential candidate solutions of a given window $w$. 
We provide the outline of SYCOS$_{\text{BU}}$ in Algorithm \ref{alg:bottomupsearch}, and explain the details below.

Given a pair of time series $(X_T,Y_T)$, and the \textit{target function} $I_w$ to be maximized, SYCOS$_{\text{BU}}$ will start with an initial solution $w=w_0$ where $\abs{w_0}=s_{\min}$ (Algorithm \ref{alg:bottomupsearch}, line $2$), and evaluate the goodness of $w$ by computing the MI $I(w_0)$ (line $3$). To maximize the target function $I_w$, SYCOS$_{\text{BU}}$ will first explore its nearest neighborhood $N_1$ and search for a better solution in this area. To do that, it computes $I(w^{'})$ for each neighbor window $w^{'} \in N_1$, and selects the best neighbor $w_{\text{best}}$ in the considered neighborhood (lines $7-11$). The best neighbor $w_{\text{best}}$ has the highest MI among all the neighbors in the same neighborhood. Then, SYCOS$_{\text{BU}}$ will determine whether $w_{\text{best}}$ is better than the current solution $w$ using the following policies:
\begin{itemize}
	\item (P1) If $I_{w_{\text{best}}} > I_w$ or $I_{w_{\text{best}}} > I_{w_h}$ where $w_h \in L_h$, then $w_{\text{best}}$ is a better solution than $w$ and thus, $w$ is replaced by $w_{\text{best}}$ (lines $13-15$).
	\item (P2) If $I_{w_{\text{best}}} < I_w$ and $I_{w_{\text{best}}} < I_{w_h}$, then there is no better solution in the considered neighborhood, and thus, no improvement can be made (lines $16-18$).
\end{itemize}

In policy P1, a better solution is found, so the search moves to this new solution $w=w_{\text{best}}$, and repeats the neighborhood exploration process on the new $w$. In policy \textit{P2}, no better solution is found, then the \textit{stopping conditions} are checked. If they are not yet satisfied, the search continues exploring a larger neighborhood. Otherwise, it stops and the value $I_w$ at the stopping point is the locally maximal value of the target function. $I_w$ is then compared to the correlation threshold $\sigma$, and $w$ is inserted into the result set $S$ if $I_w \ge \sigma$ (lines $24-26$). 

When the \textit{stopping conditions} are met and SYCOS$_{\text{BU}}$ stops, the time series might not be scanned entirely. In that case, SYCOS$_{\text{BU}}$ restarts on the remaining part of the time series, looking for new local optima, until the entire time series is searched (line $27$). 

\textit{Stopping conditions:} Ideally, SYCOS$_{\text{BU}}$ will stop immediately when no better solution can be found in the current considered neighborhood. However, to avoid situations where the occurrence of a temporary setback stops the search too early, an idle period is used to measure the number of non-improvements that has been observed. The search will stop when it reaches the pre-defined max idle period $T_{maxIdle}$ (line $6$).

\textit{Initial solution:} The first window $w_0$ of SYCOS$_{\text{BU}}$ can be at the beginning of the time series, or at an arbitrary position within the time series. In Section \ref{sec:noisetheory}, we propose a MI-based theory to select a good initial solution for SYCOS$_{\text{BU}}$.

\textit{The history list $L_h$:} SYCOS$_{\text{BU}}$ maintains a history list $L_h$ of the most recently accepted solutions and uses it to justify the goodness of a potential candidate. In our implementation, SYCOS$_{\text{BU}}$ follows the \textit{random} policy when selecting and updating an item in the history: when justifying a candidate solution, it randomly picks an element from the list and compares that element to the considered solution (line $12$); similarly, a random element from the history is selected for updating (lines $20-22$). This \textit{random} policy helps SYCOS$_{\text{BU}}$ escape \textit{plateaus} in the search space by creating the "randomness" while it moves.

\begin{algorithm}[!h]
	\small
	\caption{SYCOS$_{\text{BU}}$: Bottom-Up Search}

	\begin{algorithmic}[1]
		\Statex{{\bf Input:}} $(X_T,Y_T)$: \text{pair of time series} 
		\Statex{{\bf Params:} $\sigma$: \text{correlation threshold,}}
		\Statex{\hspace{1.23cm}$s_{\max}$: \text{maximum window size,}} 
		\Statex{\hspace{1.23cm}$s_{\min}$: \text{minimum window size}}  
		\Statex{{\bf Output:} $\mathit{S}$: \text{set of non-overlapping windows with MI $ \ge \sigma$}}
		\While{$(X_T,Y_T)$ are not completely explored}
		\State Produce an initial solution $w:=w_0$ with $\abs{w_0}=s_{\min}$ \Comment{$w_0$ can start out at the beginning or at an arbitrary location in the time series}
		\State Compute $I(w_0)$ \Comment{Evaluate the goodness of $w_0$}
		\State For all $k \in {0,...,h-1}:$ $L_{h_k}:=I(w_0)$ \Comment{Initialize the history list $L_h$ using the goodness of the initial solution}
		\State $T_{idle}:=0$ \Comment{Initialize the idle time}
		\While {$T_{idle} < T_{maxIdle}$}
		\State $N := \mathit{Neighbors}(w)$ \Comment{Identify the neighbors of $w$}
		\For  {$w^{'} \in N$}
		\State Compute $I(w^{'})$ \Comment{Evaluate the goodness of $w^{'}$} 
		\EndFor 
		\State $w_{best}:=$ \textit{BestNeighbor($N$)}\Comment{Select the best neighbor in $N$ based on the goodness measure}
		\State $w_h:=$ \textit{random.get(\textbf{$L_h$})} \Comment{Randomly select an element from the history \textbf{$L_h$}}
		\If{$I_{w_{best}}$ $>$ $I_{w_h}$ \textbf{or} $I_{w_{best}}$ $>$ $I_w$}
		\State $w:=w_{best}$ \Comment{Accept the candidate}
		\State $T_{idle}:=0$ \Comment{Reset the idle time}
		\Else 
		\State $w:=w$ \Comment{Reject the candidate}
		\State $T_{idle}:=T_{idle}+1$ \Comment{Increase the idle time}
		\EndIf
		\If{$I_w$ $>$ $I_{w_h}$}
		\State $w_{h}:=w \wedge I_{w_{h}}:=I_w$ \Comment{Update the history list}
		\EndIf
		\EndWhile
		\If{$I_w$ $\ge \sigma$}
		\State Insert $w$ to $S$ 
		\EndIf  
		\State \textit{SYCOS$_{\text{BU}}$}$(X^{'}_T,Y^{'}_T)$ \Comment{Restart SYCOS$_{\text{BU}}$ on the remaining of $(X_T,Y_T)$}
		\EndWhile
		\State \textbf{return} $S$
	\end{algorithmic}
	\label{alg:bottomupsearch}
\end{algorithm}
\normalsize






==> bottomup_bk.tex <==
\section{SYCOS$_{\text{BU}}$: Bottom-Up  Search}\label{sec:bottomup}
%We propose two approaches to search for correlated time windows: bottom-up and top-down. 
In this section, we describe the bottom-up method SYCOS$_{\text{BU}}$ that employs Late Acceptance Hill Climbing algorithm to search for correlated windows. The idea of the bottom-up search approach is to start with small-size windows, and then enlarges the window's size as the search progresses. %In contrast, the top-down approach, SYCOS$_{\text{TD}}$, starts with large-size windows, and reduces the window sizes if the series in large-size windows are not well correlated. 
This implies that SYCOS$_{\text{BU}}$ assumes correlations exist in small-size windows, and thus is more efficient to start with small windows. %Through empirical experiments in Section \ref{sec:experiment}, we show that both assumptions are valid and hold for real case studies, and depending on the case studies, one approach can be superior to another.    

\subsection{Late Acceptance Hill Climbing}
Late Acceptance Hill Climbing \cite{burke2017late}, an extension of the classic Hill Climbing (HC) \cite{russell2016artificial}, is an optimization technique attempting to find locally optimal solutions for a given problem through iterative improvement. Given a \textit{target function} $f$ and a current solution $S$ of $f$, LAHC tries to improve $S$ by exploring potential candidates in the nearby neighborhood. 
If a better solution is found (according to the predefined objectives), the current solution $S$ is replaced by this new solution $S_{\text{new}}$, and the process is repeated until no further improvement can be made.   

LAHC differs from the classic HC in its acceptance rule, i.e., it can accept a solution $S_{\text{new}}$ if $S_{\text{new}}$ is better than either the current solution $S$ or a solution $S_{\text{old}}$ found in the history. To do that, LAHC uses a fixed length array $L_h$ to maintain a history of the most recently accepted solutions, and use this $L_h$ array to justify the goodness of a candidate solution. 

One of the challenges of LAHC (or HC in general) is the convergence to \textit{local optima}. A \textit{local optimum} is a situation where the technique converges to a local best solution, but not necessarily the globally optimal one \cite{russell2016artificial}. However, in the following sections, we explain that \textit{local optima} are in fact what we are looking for in SYCOS problem.

\subsection{Apply LAHC to SYCOS}
We consider the problem of searching for synchronous correlations, i.e., SYCOS, using LAHC as a \textit{maximization} problem. Specifically, the \textit{target function} of LAHC is a \textit{maximize} function, and our goal is to search for the time windows where their MIs are locally maximal. %Thus, given a pair of time series $(X_T,Y_T)$, and the \textit{target function} $I_w=I(X_w;Y_w)$, the SYCOS problem becomes: 
%%\begin{equation}
%%\begin{split}
%%\text{SYCOS}_{\text{BU}} (X_T,Y_T) &:=\{ w_i \mid I(X_{w_i};Y_{w_i}) \ge \sigma \\&
%%\hspace{-0.5in}\wedge I(X_{w_{i-1}};Y_{w_{i-1}}) \le I(X_{w_i};Y_{w_i}) \\&
%%\hspace{-0.5in}\wedge I(X_{w_{i+1}};Y_{w_{i+1}}) \le I(X_{w_{i}};Y_{w_{i}})
%%\} 
%%\end{split}
%%\label{eq:pbformulation}
%%\end{equation}
%%Eq. \ref{eq:pbformulation} represents a set of all windows $w_i$ whose MIs are locally maximal values that satisfy the correlation threshold.  
%\textit{Why are local optima the solutions of SYCOS$_{\text{BU}}$?}
 %is LAHC a good candidate solution for correlation search?}}
To explain why local optima are in fact the solutions of SYCOS$_{\text{BU}}$, consider Fig. \ref{fig:mifluctuation} that plots the fluctuation of MI values for a given pair of variables. Here, the $y-$axis represents the MI values of the time windows on the $x-$axis. Given the correlation threshold $\sigma$ (red line in Fig. \ref{fig:mifluctuation}), the three windows which correspond to the three maximal points (in red) indicate highly correlated areas (above $\sigma$). %the search will extract three different windows which correspond to three maximal points (in red) which is above $\sigma$
These windows can be found by first identifying the three peak points which represent the locally maximal MI values, and then extending the located points to the surrounding areas to determine the precise window's indices. Such windows are guaranteed to satisfy the correlation condition: $I_w \ge \sigma$. 

\begin{figure}[!h]
	\vspace{-0.12in}
	\centering
	\includegraphics[width=0.35\textwidth]{figures/MIFluctuation2D} %{figures/MI1} {figures/MI2}
	\vspace{-0.1in}
	\caption{Mutual information fluctuation}
	\label{fig:mifluctuation}
	\vspace{-0.1in}
\end{figure}
%Since an LAHC-based method guarantees local optimal solutions, it is an ideal solution for SYCOS. % for general problems, and global optimal solutions for convex problems \textbf{need citation}. %– otherwise it will find only local optima (solutions that cannot be improved by considering a neighboring configuration), which are not necessarily the best possible solution (the global optimum) out of all possible solutions (the search space). Examples of algorithms that solve convex problems by hill-climbing include the simplex algorithm for linear programming and binary search.[1]:253 To attempt overcoming being stuck in local optima, one could use restarts (i.e. repeated local search), or more complex schemes based on iterations (like iterated local search), or on memory (like reactive search optimization and tabu search), or on memory-less stochastic modifications (like simulated annealing).
%The property to guarantee local optimal solutions makes Hill Climbing a perfect candidate to search for temporal correlations in time series. We explain how this property makes the method a perfect candidate for correlation search in the next section. %Other properties such as the simplicity and the ability to provide valid solution at anytime make the algorithm a popular choice amongst other optimization algorithms. 
%\textit{Why finding local optima is a good property for temporal correlation search?} because finding correlations in time series means to maximize the MI within a certain time duration, which implies the local optimal among the entire time series.

%Indeed, finding correlations in time series means to find the time windows that maximize the MI, which implies finding the locally optimal solutions that are above the correlation threshold.
Since an LAHC-based method guarantees local optimal solutions, it is an ideal technique for SYCOS. Moreover, during the search process, an LAHC-based method does not maintain a complete search tree since it looks only at the current state and neighbor states, thus is memory efficient. %This is another advantage of using LAHC-based methods for correlations search. % in big time series. 

\textit{Definition 5.1} \textit{($\delta$-neighbor)} Let $(X_T,Y_T)$ be a pair of time series of length $n$ measured during the time interval $T$, and $w=[t_s,t_e]$ be a time window of $(X_T,Y_T)$. A window $w^{'}=[t_s^{'},t_e^{'}]$ is an \textit{$\delta$-neighbor} of $w$ if $(t_s^{'}=t_s-\delta$ $\vee$ $t_s^{'}=t_s+\delta)$  $\vee$ $(t_e^{'}=t_e-\delta$ $\vee$ $t_e^{'}=t_e+\delta)$, where $\delta$ is a pre-defined moving step such that $1 \le \delta \le n$ $\wedge$ $s_{\min} \le \abs{w^{'}} \le s_{\max}$. 
\\
\textit{Definition 5.2} \textit{($\delta$-neighborhood)} Let $w=[t_s,t_e]$ be a time window of $(X_T,Y_T)$. A \textit{$\delta$-neighborhood} $N$ of $w$, denoted as $N_{\delta}$, is the surrounding area of $w$ formed by all \textit{$\delta$-neighbors} $w^{'}=[t_s^{'},t_e^{'}]$ of $w$. 

\begin{figure}[!h]
	\centering
	\resizebox{.7\linewidth}{!}{
	\begin{tikzpicture}%[scale=0.8]
	\begin{axis}[inner axis line style={black},
	axis lines=center,axis line style={-latex},
	tick style={draw=none},
	ymin = 0, ymax = 15,
	xmin = 0, xmax = 12,
	xscale=1.3,
	xticklabels={,,},
	yticklabels={,,},
	xlabel=$t_s$,
	ylabel=$t_e$,
	xlabel style={
		at={(ticklabel cs:0.95)},
		anchor=west,
	},
	ylabel style={
		at={(ticklabel cs:0.95)},
		anchor=south,
	}
	]
	\coordinate (O) at (axis cs:0,0);
	\coordinate (X) at (axis cs:1,0);
	\coordinate (Y) at (axis cs:0,1);
	\end{axis}  
	\begin{scope}[x={($(X)-(O)$)}, y={($(Y)-(O)$)}, shift={(O)}]
	
	
	\foreach \v in {1,2,...,\cols} {
		\pgfmathsetmacro{\ynew}{(1+(\v-1)*\kcachy)}
		\drawdot{black}{\v}{\ynew}{\rows}{\kcach}; 
	};
	
	\foreach \v in {1,2,...,\rows} {
		\draw [black] (1, {(1+(\v-1)*\kcach)}) -- (\cols, {(1+(\cols-1)*\kcachy)+(\v-1)*\kcach)});
	};
	
	\foreach \v in {3,4,...,7} {
		\pgfmathsetmacro{\Y}{(1+(\v-1)*\kcachy)}
		\pgfmathsetmacro{\ynew}{(\Y+\kcach)}
		\drawdot{blizzardblue}{\v}{\ynew}{5}{\kcach}; 
	};
	
	\foreach \v in {4,5,6} {
		\pgfmathsetmacro{\Y}{(1+(\v-1)*\kcachy)}
		\pgfmathsetmacro{\ynew}{(\Y+2*\kcach)}
		\drawdot{blue-violet}{\v}{\ynew}{3}{\kcach}; 
	};
	\node [circle,draw=black, fill=blue, scale=0.6] (center) at (5, {(1+4*\kcachy+3*\kcach)}) {};
	
	\draw [black, dashed] (0,1) -- (1,1);
	\draw [black, dashed] (0,{(1+(\rows-1)*\kcach)}) -- (1,{(1+(\rows-1)*\kcach)});
	\draw [black, dashed] (1,0) -- (1,1);
	\draw [black, dashed] (0,{((1+(\cols-1)*\kcachy)+(\rows-1)*\kcach)}) -- (\cols,{((1+(\cols-1)*\kcachy)+(\rows-1)*\kcach)});
	\draw [black, dashed] (\cols,0) -- (\cols,{((1+(\cols-1)*\kcachy)});
	
	\node [red] at (-0.6,1) {\small $t_{e_{11}}$};
	\node [red] at (-0.6,{(1+(\rows-1)*\kcach)}) {\small $t_{e_{1l}}$};
	
	\node [red] at (1,-0.6) {\small $t_{s_{1}}$};
	\node [blue] at (\cols,-0.6) {\small $t_{s_{m}}$};
	
	\node [blue] at (\cols+1,{((1+(\cols-1)*\kcachy)}) {\small $t_{e_{m1}}$};
	\node [blue] at (\cols+1,{((1+(\cols-1)*\kcachy)+(\rows-1)*\kcach)}) {\small $t_{e_{ml}}$};
	
	\node [blue] (iw) at (-0.9,7) {$I_w$};
	\draw [-latex, dashed, blue] (iw) -- (center);
	
	\node [blue] at (5.4, {(1+4*\kcachy+1*\kcach)+0.6}) {\tiny $W^b_{N2}$};
	\node [blue] at (5.4, {(1+4*\kcachy+2*\kcach)+0.6}) {\tiny $W^b_{N1}$};
	\node [blue] at (5.4, {(1+4*\kcachy+4*\kcach)+0.6}) {\tiny $W^t_{N1}$};
	\node [blue] at (5.4, {(1+4*\kcachy+5*\kcach)+0.6}) {\tiny $W^t_{N2}$};
	
	\node [blue] at (5.2, {(1+4*\kcachy+3*\kcach)+0.6}) {\tiny $W$};
	
	\node [blue] at (3.4, {(1+3*\kcachy+3*\kcach)-0.7}) {\tiny $W^l_{N2}$};
	\node [blue] at (4.4, {(1+4*\kcachy+3*\kcach)-0.7}) {\tiny $W^l_{N1}$};
	\node [blue] at (6.4, {(1+6*\kcachy+3*\kcach)-0.7}) {\tiny $W^r_{N1}$};
	\node [blue] at (7.4, {(1+7*\kcachy+3*\kcach)-0.7}) {\tiny $W^r_{N2}$};

	\end{scope}
	\end{tikzpicture}
}
\vspace{-0.1in}
\caption{Search space for SYCOS$_{\text{BU}}$}
\label{fig:searchspacebf}
\end{figure}

%%\begin{figure}[!h]
%%	\centering
%%	\includegraphics[width=0.35\textwidth]{figures/bruteforce_new}
%%	\vspace{-0.1in}
%%	\caption{Search space for SYCOS$_{\text{BU}}$ \textbf{to fix the missing lines}}
%%	\label{fig:searchspacebf}
%%\end{figure}

We illustrate the \textit{neighborhood} concept in Fig. \ref{fig:searchspacebf}. % that represents the search space of SYCOS$_{\text{BU}}$. 
Here, each point in the grid represents a time window with the x-axis represents the start time, and the y-axis represents the end time. Consider the window $w$ in blue. The nearest $\delta-$neighborhood of $w$, called the $1-$neighborhood $N_1$, is the area formed by the \textit{eight} windows in light purple color surrounding $w$. Each window in this neighborhood differs from $w$ by \textit{one} $\delta$ step, either by its start index, or its end index, or both. Going further from $w$, the next neighborhood of $w$, called the $2-$neighborhood $N_2$, is the $16$ windows in light blue color. Each $\delta-$\textit{neighborhood} will form an area where LAHC will iteratively look for potential candidate solutions of a given window $w$. 
We provide the outline of SYCOS$_{\text{BU}}$ in Algorithm \ref{alg:bottomupsearch}, and explain the details below.

Given a pair of time series $(X_T,Y_T)$, and the \textit{target function} $I_w$ to be maximized, SYCOS$_{\text{BU}}$ will start with an initial solution $w=w_0$ where $\abs{w_0}=s_{\min}$ (Algorithm \ref{alg:bottomupsearch}, line $2$), and evaluate the goodness of $w$ by computing the MI $I(w_0)$ (line $3$). To maximize the target function $I_w$, SYCOS$_{\text{BU}}$ will first explore its nearest neighborhood $N_1$ and search for a better solution in this area. To do that, it computes $I(w^{'})$ for each neighbor window $w^{'} \in N_1$, and selects the best neighbor $w_{\text{best}}$ in the considered neighborhood (lines $7-11$). The best neighbor $w_{\text{best}}$ has the highest MI among all the neighbors in the same neighborhood. Then, SYCOS$_{\text{BU}}$ will determine whether $w_{\text{best}}$ is better than the current solution $w$ using the following policies:
\begin{itemize}
	\item (P1) If $I_{w_{\text{best}}} > I_w$ or $I_{w_{\text{best}}} > I_{w_h}$ where $w_h \in L_h$, then $w_{\text{best}}$ is a better solution than $w$ and thus, $w$ is replaced by $w_{\text{best}}$ (lines $13-15$).
	\item (P2) If $I_{w_{\text{best}}} < I_w$ and $I_{w_{\text{best}}} < I_{w_h}$, then there is no better solution in the considered neighborhood, and thus, no improvement can be made (lines $16-18$).
\end{itemize}

In policy P1, a better solution is found, so the search moves to this new solution $w=w_{\text{best}}$, and repeats the neighborhood exploration process on the new $w$. In policy \textit{P2}, no better solution is found, then the \textit{stopping conditions} are checked. If they are not yet satisfied, the search continues exploring a larger neighborhood. Otherwise, it stops and the value $I_w$ at the stopping point is the locally maximal value of the target function. $I_w$ is then compared to the correlation threshold $\sigma$, and $w$ is inserted into the result set $S$ if $I_w \ge \sigma$ (lines $24-26$). 

When the \textit{stopping conditions} are met and SYCOS$_{\text{BU}}$ stops, the time series might not be scanned entirely. In that case, SYCOS$_{\text{BU}}$ restarts on the remaining part of the time series, looking for new local optima, until the entire time series is searched (line $27$). 

\textit{Stopping conditions:} Ideally, SYCOS$_{\text{BU}}$ will stop immediately when no better solution can be found in the current considered neighborhood. However, to avoid situations where the occurrence of a temporary setback stops the search too early, an idle period is used to measure the number of non-improvements that has been observed. The search will stop when it reaches the pre-defined max idle period $T_{maxIdle}$ (line $6$).

\textit{Initial solution:} The first window $w_0$ of SYCOS$_{\text{BU}}$ can be at the beginning of the time series, or at an arbitrary position within the time series. In Section \ref{sec:noisetheory}, we propose a MI-based theory to select a good initial solution for SYCOS$_{\text{BU}}$.

\textit{The history list $L_h$:} SYCOS$_{\text{BU}}$ maintains a history list $L_h$ of the most recently accepted solutions and uses it to justify the goodness of a potential candidate. In our implementation, SYCOS$_{\text{BU}}$ follows the \textit{random} policy when selecting and updating an item in the history: when justifying a candidate solution, it randomly picks an element from the list and compares that element to the considered solution (line $12$); similarly, a random element from the history is selected for updating (lines $20-22$). This \textit{random} policy helps SYCOS$_{\text{BU}}$ escape \textit{plateaus} in the search space by creating the "randomness" while it moves.

\begin{algorithm}[!h]
	\small
	\caption{SYCOS$_{\text{BU}}$: Bottom-Up Search}

	\begin{algorithmic}[1]
		\Statex{{\bf Input:}} $(X_T,Y_T)$: \text{pair of time series} 
		\Statex{{\bf Params:} $\sigma$: \text{correlation threshold,}}
		\Statex{\hspace{1.23cm}$s_{\max}$: \text{maximum window size,}} 
		\Statex{\hspace{1.23cm}$s_{\min}$: \text{minimum window size}}  
		\Statex{{\bf Output:} $\mathit{S}$: \text{set of non-overlapping windows with MI $ \ge \sigma$}}
		\While{$(X_T,Y_T)$ are not completely explored}
		\State Produce an initial solution $w:=w_0$ with $\abs{w_0}=s_{\min}$ \Comment{$w_0$ can start out at the beginning or at an arbitrary location in the time series}
		\State Compute $I(w_0)$ \Comment{Evaluate the goodness of $w_0$}
		\State For all $k \in {0,...,h-1}:$ $L_{h_k}:=I(w_0)$ \Comment{Initialize the history list $L_h$ using the goodness of the initial solution}
		\State $T_{idle}:=0$ \Comment{Initialize the idle time}
		\While {$T_{idle} < T_{maxIdle}$}
		\State $N := \mathit{Neighbors}(w)$ \Comment{Identify the neighbors of $w$}
		\For  {$w^{'} \in N$}
		\State Compute $I(w^{'})$ \Comment{Evaluate the goodness of $w^{'}$} 
		\EndFor 
		\State $w_{best}:=$ \textit{BestNeighbor($N$)}\Comment{Select the best neighbor in $N$ based on the goodness measure}
		\State $w_h:=$ \textit{random.get(\textbf{$L_h$})} \Comment{Randomly select an element from the history \textbf{$L_h$}}
		\If{$I_{w_{best}}$ $>$ $I_{w_h}$ \textbf{or} $I_{w_{best}}$ $>$ $I_w$}
		\State $w:=w_{best}$ \Comment{Accept the candidate}
		\State $T_{idle}:=0$ \Comment{Reset the idle time}
		\Else 
		\State $w:=w$ \Comment{Reject the candidate}
		\State $T_{idle}:=T_{idle}+1$ \Comment{Increase the idle time}
		\EndIf
		\If{$I_w$ $>$ $I_{w_h}$}
		\State $w_{h}:=w \wedge I_{w_{h}}:=I_w$ \Comment{Update the history list}
		\EndIf
		\EndWhile
		\If{$I_w$ $\ge \sigma$}
		\State Insert $w$ to $S$ 
		\EndIf  
		\State \textit{SYCOS$_{\text{BU}}$}$(X^{'}_T,Y^{'}_T)$ \Comment{Restart SYCOS$_{\text{BU}}$ on the remaining of $(X_T,Y_T)$}
		\EndWhile
		\State \textbf{return} $S$
	\end{algorithmic}
	\label{alg:bottomupsearch}
\end{algorithm}
\normalsize






==> implementation.tex <==
\subsection{Incremental MI Computation}\label{sec:implementation}
In the previous sections, we discuss how to use the noise theory to reduce the search space of the bottom-up and the top-down approaches. In this section, we propose another improvement to efficiently compute the MI values across nearby windows. 

\subsection{Box-assisted algorithm}
Recall that to compute the MI of a window, the \textit{KSG} estimator needs to estimate the population density of data points in that window. To do that, for each data point $p_i=(x_i,y_i)$ in the considered window, it first searches for the $k$ nearest neighbors of $p_i$, and then counts the number of marginal points $n_x$, $n_y$ that fall into the marginal $k$-nearest distances in each dimension $d_x$, $d_y$ \cite{kraskov2004estimating}. 
Among all the computations, $k$-nearest neighbor (\textit{knn}) search is the most expensive operator. Therefore, we design an efficient data structure to optimize the \textit{knn} search using the boxed-assisted method \cite{vejmelka2007mutual}. %Note that the boxed-assisted method has been shown to outperform other methods (e.g., k-D tree, projection method) in \textit{knn} search for low dimensional data \cite{vejmelka2007mutual}. 

In the box-assisted method, the search space is divided into equal size boxes where each data point is projected into exactly one box. Each box maintains a list of points belonging to that box. When searching for the $k$-nearest neighbors of point $p_i$, first the box containing $p_i$ is found. Then, the search starts from that box and extends to nearby boxes to find the $k$ nearest points. Next, the distances to the $k^{\text{th}}$-neighbor in each dimension $d_x$, $d_y$ are determined, and the marginal points $n_x$, $n_y$ are computed by counting the number of points falling within these distances. The values of $n_x$ and $n_y$ will then be used in Eq. \ref{formula:KSGmi} to estimate the final MI value.

Fig. \ref{fig:influencedregion1} illustrates the boxed-assisted method and how it is used in KSG to compute the MI of a window that contains $7$ data points $p_1,...,p_7$. Consider point $p_1$ (red) in the figure. Assume that $k=2$ is nearest neighbor parameter, and \textit{maximum norm}\footnote{\small $L_{\infty}$: $d(p_i,p_j)=\parallel (d_x,d_y) \parallel_{\max}=\max(\parallel x_i-x_j\parallel,\parallel y_i-y_j\parallel)$} is the distance metric. In this setting, the two nearest neighbors of $p_1$ are $p_2$ and $p_3$ (green), and the nearest distances in each dimension are $dx$ and $dy$ (shown in the figure). The nearest distances allow KSG to form the marginal regions (in gray shade), from which the marginal counts are computed. In this case, for point $p_1$, the marginal counts are $n_x=3$ (including $p_2,p_3,p_5$), and $n_y=3$ (including  $p_2,p_3,p_4$). A similar process is applied to other points in the window, and the final MI is computed by accumulating the obtained $n_x$ and $n_y$ values.

\begin{figure}[!t]
	\centering
	\begin{subfigure}{.24\textwidth}
		\includegraphics[width=0.9\linewidth]{Figures/influence_region_1}	
		\caption{\footnotesize{Box-assisted method}}
		\label{fig:influencedregion1}
	\end{subfigure}
	\begin{subfigure}{.24\textwidth}
		\includegraphics[width=0.9\linewidth]{Figures/influence_region_2}
		\caption{\footnotesize{IR (green) and IMR (gray)}}
		\label{fig:influencedregion2}
	\end{subfigure}
	\caption{Efficient and incremental MI computation} 
	\label{fig:influencedregion}
\end{figure}

\subsection{Incremental MI computation with influenced regions}
We showed above how the noise theory could reduce revisiting the same data partition.  However, it is still possible that nearby windows share the same data. For example, in Fig. \ref{fig:searchspacebf}, when SYCOS$_{\text{BU}}$ moves leftwards, the neighbor window $w^{l}_{N1}=w_\delta  \odot w$ is formed by adding a new data partition $w_\delta$ to the current window $w$. Here, the shared data between $w$ and $w^{l}_{N1}$ are exactly $w$ itself. % by just a data partition $w_\delta$ which is the newly added data to $w$. Similarly for rightwards, upwards, downwards exploration directions. %$w^{t}_{N1}=w \odot w_\delta$. Rightwards, $w^{r}_{N1}=w\setminus w_\delta$, where $w_\delta$, in this case, is the data being removed from $w$. In a similar way, $w^{b}_{N1}$ is created by removing a part of data from $w$. These neighbors, in fact, differ from $w$ by only a small data partition $w_\delta$. Thus, ideally, the computation of $w$ should be reused. To do that, we design an optimized boxed-assisted algorithm to ensure only new data in the considered window need to be computed, and only data affected by the changes (introduced by removing data or by adding new data) are re-evaluated. 
Similarly, in SYCOS$_{\text{TD}}$, the shifting from $w_1$ to $w_2$ in Fig. \ref{fig:topdownsearchtree} creates three different groups of data: \textit{Group 1} from $s_1$ to $s_2$ contains the data points of $w_1$  to be removed from $w_2$, \textit{Group 2} from $s_2$ to $e_1$ is overlapping data between $w_1$ and $w_2$, and \textit{Group 3} from $e_1$ to $e_2$ is newly added data to $w_2$. Ideally, computations on overlapping data should be reused. To do that, we design an optimized boxed-assisted method to ensure that computation is only done on new data. On overlapping data, only those affected by changes (by removing or adding data) are re-evaluated. 
%To minimize the computation cost, we design an optimized boxed-assisted algorithm to track changes introduced by removing old data ($[s_1,s_2]$) and by adding new data ($[e_1,e_2]$). The optimization ensures that for each new window $w_2$, only new data need to be computed, and only data affected by the changes are re-evaluated. 
%Thus, ideally, the computation of $w$ should be reused. To do that, we design an optimized boxed-assisted algorithm to ensure only new data in the considered window need to be computed, and only data affected by the changes (introduced by removing data or by adding new data) are re-evaluated. 
%In addition to the boxed-array used in the standard version, we use additional data structures to keep track of the previous computation (e.g., of $w_1$). For each data point $i$, we add 3 components to its data structure to store: (1) the index of the $k^{\text{th}}$-nearest neighbor, (2) the distance in each dimension to its $k^{\text{th}}$-nearest neighbor, (3) the number of marginal points in each dimension.
Note that the introduced changes can be either change the $k$-nearest neighbors of existing points or the marginal counts $n_x$, $n_y$. To keep track of the previous computation, we introduce the concepts of \textit{influenced region} and \textit{influenced marginal region}.

\textit{Definition 10.1} An \textit{influenced region} (\textit{IR}) of point $p_i=(x_i,y_i)$ is a square bounding box $R_{i}=(l_{i},r_{i},b_{i},t_{i})$, where $l_{i},r_{i},b_{i},t_{i}$ are its left-, right-, bottom-, and top-most indices, respectively, which are computed as $l_{i}=x_i-d$, $r_{i}=x_i+d$, $b_{i}=y_i+d$, $t_{i}=y_i-d$ where $d=\max(d_x,d_y)$.

\textit{Definition 10.2} The \textit{influenced marginal region(s)} (\textit{IMR}) of point $p_i$ is (are) the marginal region(s) located within the nearest distance $d_i$ in each dimension. 

Fig. \ref{fig:influencedregion2} illustrates the \textit{influenced region} and \textit{influenced marginal region} concepts. The \textit{influenced region} of $p_1$ is the square colored in green, and the \textit{influenced marginal regions} are those with gray shade in either dimension. 

\begin{lem}\label{lem3}
	Given a window $w_i$ and a data point $p \in w_i$, a new point $o$ inserted into $w_i$ will become the new $k^{th}$-neighbor of $p$ iff $o$ is within IR of $p$. 
	\vspace{-0.08in}
\end{lem}

\begin{lem}\label{lem4}
	Given a window $w_i$ and a data point $p \in w_i$, an existing point $o$ deleted from $w_i$ will change the $k$ nearest points of $p$ iff $o$ is within IR of $p$. 
	\vspace{-0.08in}
\end{lem}

\begin{lem}\label{lem5}
	Given a window $w_i$ and a data point $p \in w_i$, a new point $o$ inserted into $w_i$ will increase the marginal count $n_x$ (or $n_y$) of $p$ iff $o$ is within \textit{IMR}$_x$ (or \textit{IMR}$_y$) of $p$.
	\vspace{-0.08in}
\end{lem}

\begin{lem}\label{lem6}
	Given a window $w_i$ and a data point $p \in w_i$, an existing point $o$ deleted from $w_i$ will reduce the marginal count $n_x$ (or $n_y$) of $p$ iff $o$ is within \textit{IMR}$_x$ (or \textit{IMR}$_y$) of $p$.
	\vspace{-0.08in}
\end{lem}

\begin{proof}
	Proofs of Lemmas \ref{lem3}, \ref{lem4}, \ref{lem5}, \ref{lem6} are straightforward, thus omitted.   
\end{proof}

Lemmas \ref{lem3}, \ref{lem4}, \ref{lem5}, \ref{lem6} display unique properties of \textit{IRs} and \textit{IMRs}. An \textit{IR} maintains an area where any point $p_j$ either being added to or removed from this region will change the $k$ nearest points of $p_i$. In this case, a new $k$-nearest neighbors search is required for $p_i$. Instead, an \textit{IMR} maintains an area where any point $p_j$ either being added to or removed from it will change the marginal counts of $p_i$. In this case, the marginalized neighbors of $p_i$ have to be recounted. 

Fig. \ref{fig:influencedregion2} illustrates how changes are introduced and managed. For simplicity, we only discuss the cases when new points are added into a previous computation. Changes introduced by removing points can be handled in a similar way. Assume that at time $t_1$, a new point $p_8$  is added to the current window and falls into the IR of $p_1$. The addition of $p_8$ changes the $k^{th}$-nearest neighbor of $p_1$. Thus, a new nearest neighbor search for $p_1$ is required. 

At time $t_2$, a new point $p_9$ arrives and falls into the $y$-marginal influenced region of $p_1$, for which it will alter the marginal count $n_y$  (but no new $k$-nearest neighbor search is required in this case). Similarly, a new point $p_10$ will increase the marginal count $n_x$. In these cases, only a recount of $n_x$ or $n_y$ is performed. 

As the result of our \textit{optimized box-assisted computation} method, for each window, only a minimum search region (containing new points) and a minimum update region (containing points affected by added and removed points) require additional computation. The rest is reused, thus minimizing the computational cost.



==> introduction-new.tex <==
\section{Introduction}

% \textbf{Old introduction below}

% Motivations and examples
Recent advancements in IoT technology enable the collection of enormous amounts of time series data at unprecedented scale and speed across different domains. The availability of these massive and heterogeneous datasets offers rich  opportunities to extract insights and uncover hidden patterns and relationships between seemingly separated events and/or phenomenons via data analytics. One of the first and crucial steps in performing data analytics is to discover correlations among heterogeneous and cross-domain datasets.

% For example, a modern wind turbine has hundreds of sensors sampled at a high frequency, a smart building contains thousands of sensors sensing the surrounding environment, an autonomic vehicle carries numerous vision sensors, all of them are collecting terabytes of data every day.

Consider for example urban datasets such as the NYC Open Data \cite{nycopen} with more than 1,500 published datasets containing quantitative data from a wide range of different domains, including weather and transportation, energy and environment, education and business etc.. Crossed analysis among these datasets can reveal new insights about the city and its citizens, and thus aid policy makers as well as urban planners in decision making. 
%
For instance, correlations between weather and transportation data can identify weather events or patterns, such as a storm or prolong heavy rain, which can help provide the explanation for an abnormal increase in the number of traffic accidents. 
%
Correlations between weather data and energy production and/or consumption data can provide an accurate prediction of the city's energy capacity and need at a specific point in time, thus allowing better resources planning. 
%
Data correlation in the financial domain can help forecast the price movement of stocks or predict the purchasing behavior of consumers, and thus assist investors in making real-time investment decisions. 
%
Not only useful in reasoning and predicting, data correlation can also be considered as one of the three building blocks to establish a causal relation \cite{agresti2012social}, and thus can serve as a basis for constructing inference and learning models. 

% \textit{Challenges and current limitations:}
\subsection{State of the art and research challenges {\bf need inputs from Ngyen}}
{\bf Want to highlight 3 main changlenges here: (1) varying temporal scale, (2) non-linear relationship, and (3) noise. Want to discuss each challenge in more detail and provide prior work or lack thereof if possible.}
           
Despite its promising potentials, finding correlation in big and heterogeneous time series datasets is challenging. Not only does the huge volume of data raise significant challenges in terms of performance and scalability, their varying time scale and noisy nature also presents difficulties in finding different types of correlation relations, or in the ability to deal with adaptive temporal scales.
%
Cross-domain correlations often appear at different temporal scales. For example, correlations involving weather data might span over multiple temporal scales ranging from hours (e.g., during rain showers), to days, or even weeks (e.g., during a storm) depending on the weather events.
%
Furthermore, real-world datasets also exhibit different types of correlation, including linear and non-linear, monotonic and non-monotonic, functional and non-functional. Numerous datasets, such as stock prices or weather information, exhibit non-linear relations, which rule out the use of traditional linear correlation measures such as the Pearson coefficients \cite{kenney2013mathematics}.
{\bf Are there other prior works on finding correlation? Should mention and discuss them here. }
These datasets are also inherently noisy with varying noise levels depending on the type of data and the method of collection. This noise presents a challenge for robust algorithms. {\bf Any prior work or comments on the lack thereof on dealing with noisy data?} 

Although correlation search has been studied extensively in the literature, current state-of-the-art techniques are limited either in the type of detected relations, focusing only on linear ones \cite{}, or in the temporal scale they consider. Most of the correlation works do not consider adaptive temporal scales as they assume that correlations only exist for a fixed time period, e.g., \cite{bermudez2018analysing,shakil2018parametric}. Thus these existing methods can be inefficient for performing correlation search in big, complex, and cross-domain time series data where multiple temporal scales exist.

{\bf Review of other related concepts but not the same -- any concepts other than similarity? can include that here too. }
Moreover, there is often a misconception that correlations and similarities in time series are the same, where in fact, they are two different concepts. Correlations refer to statistical relationships present in the data, whereas similarities mean to find the optimal matching and/or alignment between the time series sequences.
{\bf This difference can be explained / developed in more detail as this sentence is still a bit vague -- what is optimal matching or alignment? how is it different from statistical relationship? }
Thus methods such as Dynamic Time Warping \cite{salvador2007toward} may not be suitable for correlation search.

The idea of the bottom-up search method SYCOS$_{\text{BU}}$ is to start with small-size windows, and then extends the window sizes as the search progresses. In contrast, the top-down approach, SYCOS$_{\text{TD}}$, starts with large-size windows, and reduces the window sizes if the series in large-size windows are not well correlated. 
Intuitively, SYCOS$_{\text{BU}}$ assumes that correlations exist in small-size windows, while SYCOS$_{\text{TD}}$ assumes the opposite. Through empirical experiments in Section \ref{sec:experiment}, we show that both assumptions are valid and hold for real case studies, and depending on the case studies, one approach can be superior to another.    

% \textit{Contributions:}
\subsection{Our contributions}
This paper aims to address challenges identified above, namely (1) varying temporal scale, (2) non-linear relationship, and (3) noisy data, by introducing the SYnchronous COrrelation Search (SYCOS) approach to search for synchronous correlations in big time series data, making the following novel contributions: 

\begin{itemize}
	\item 	SYCOS searches for correlation based on mutual information between different data windows. The measure of mutual information is robust to noise and underlying data distributions, and is able to capture various types of correlation relations, including linear and non-linear, monotonic and non-monotonic, functional and non-functional. Mutual information can also be computed for windows of any size, making it adaptive to varying temporal scales.
	\item   Using mutual information as the metric in the well-known Late Acceptance Hill Climbing (LAHC) search method with a window-based approach, SYCOS can automatically discover correlations at multiple temporal scales without requiring user inputs to specify the time scales or window sizes. The window sizes are automatically adjusted based on mutual information values which indicate a potential correlation.
        \item  We propose two window-based search methods, a top-down and a bottom-up, for finding correlation in different types of data. The top-down approach starts with the largest window size and gradually narrows down the size for increasing correlations and is suitable for datasets containing correlation across large time scales. On the contrary, the bottom-up approach starts with the smallest window granularity and increases the window size until mutual information increment diminishes. The bottom-up approach is suitable for datasets where correlations are expected in small bursts of data.
	\item  Based on probability theory, we propose a novel method to threshold the noise level in the process of computing mutual information, hence enabling efficient pruning of non-interesting time intervals from the search and significantly reducing the search space and improving the search speed. This effective noise threshold also improves the robustness of our proposed approaches in processing noisy data.
	\item  SYCOS employs an optimization engine to reuse mutual information computation across a large number of neighboring windows, thus minimizing computation redundancy and improving speed. This optimization makes SYCOS scalable and memory efficient in both the top-down and bottom-up approaches and therefore suitable for big datasets.
	\item  We perform a comprehensive experimental evaluation of both approaches using synthetic and real-world datasets from the energy and smart city domains. Experiment results show that SYCOS is able to find important correlations among these time series with high accuracy and is up to an order of magnitude faster than state-of-the-art techniques.
	
	And finally, we perform an extensive experimental comparison between SYCOS$_{\text{TD}}$ and SYCOS$_{\text{BU}}$ to show that SYCOS framework can select the most efficient method for a given input. This experimental analysis shows that our unified SYCOS method combines the strengths of both SYCOS$_{\text{BU}}$ and SYCOS$_{\text{TD}}$, and provides a holistic robust correlation search solution for all types of data.  
	
	 {\bf May want to add a comment or conclusion on the comparison between the top-down and bottom-up approaches here.}
\end{itemize}




==> introduction.tex <==
\section{Introduction}

\textbf{Old introduction below}

Recent developments in IoT technology have enabled the collection of enormous amounts of time series data at unprecedented scale and speed. For example, a modern wind turbine has hundreds of sensors sampled at a high frequency, a smart building contains thousands of sensors sensing the surrounding environment, an autonomic vehicle carries numerous vision sensors, all of them are collecting terabytes of data every day. The availability of these massive, heterogeneous and rich datasets opens opportunities to extract new insights, uncover hidden patterns, and support evidence-based decision making. 

To harness the enormous value from such big time series, one of the first steps is to discover correlations among heterogeneous and cross-domain datasets. Consider for example the NYC Open Data \cite{nycopen} with more than 1,500 published datasets containing quantitative data from a wide range of different domains, including weather and transportation, energy and environment, education and business etc., crossed analysis among these datasets can reveal new insights about the city and its citizens, and thus aid policy makers in decision making. 
For instance, finding correlations between weather and transportation data can lead to the identification of individual weather events, such as the occurrence of a storm or a hurricane, which can help provide the explanation for an abnormal increase in the number of accidents. 
Data correlation is also useful in behavioral predicting and future planning. For example, illustrating that weather data (e.g., wind speed or solar radiance) is well-correlated with energy production can provide accurate prediction of the city's energy capacity at a specific point in time, thus allowing better resources planning. 
In the financial domain, data correlation can help forecast the price movement of related stocks, or predict the purchasing behavior of consumers, and thus assist investors in making real-time investment decisions. 
Not only is it useful in reasoning and predicting, data correlation can also be considered as one of the three building blocks to establish a causal relation \cite{agresti2012social}, and thus can serve as a basis for constructing inference and learning models. 

\textit{Challenges and current limitations:} Despite its potential use, finding correlations in big and heterogeneous time series datasets is challenging. Not only does the very large volume of data raise significant challenges in terms of performance and scalability, their complex and noisy nature also presents difficulties in finding different types of correlation relations, or in the ability to deal with adaptive temporal scales. For example, stock prices or weather information exhibit non-linear relations, which rule out the use of traditional correlation measures such as the Pearson correlation coefficients \cite{kenney2013mathematics} which can only capture linear ones. Moreover, there is often a misconception that finding correlations and finding similarities in time series are the same task, where in fact, they are two different problems. Finding correlations is to look for statistical relationships present in the data, whereas finding similarities means to find the optimal matching and/or alignment between the time series sequences. This therefore excludes methods such as Dynamic Time Warping \cite{salvador2007toward} from the set of potential solutions for correlation search.  

To make the problem even more challenging, cross-domain correlations might appear at different temporal scales. As an example, correlations involving weather data might span over multiple temporal scales ranging from hours (e.g., during rain showers), to days, or even weeks (e.g., during a storm) depending on the weather events. Finding correlations in a Big Data context thus requires not only a robust correlation measure that can capture different types of relations (e.g., linear vs. non-linear, functional vs. non-functional, monotonic vs. non-monotonic), but also a method that can identify  multi-temporal scale correlations. 

Although correlation search has been studied extensively in the literature, current state-of-the-art techniques are limited either in the type of detected relations, i.e., only linear ones, or in the temporal scale which they deal with. Most of the correlation works do not consider adaptive temporal scales as they assume that correlations only exist for a fixed time period, e.g., \cite{bermudez2018analysing,shakil2018parametric}. Thus these existing methods are not suitable for performing correlation search in big, complex, and cross-domain time series data. 

\textit{Contributions:}
This paper aims to address these challenges and limitations by introducing the SYnchronous COrrelation Search (SYCOS) approach to search for synchronous correlations in big time series data, making the following novel contributions: 

\begin{itemize}
	\item 	SYCOS is based on the concept of mutual information from information theory, giving it a strong theoretical foundation and the ability to discover various types of correlation relations, including linear and non-linear, monotonic and non-monotonic, functional and non-functional.
	\item   By combining the well-known Late Acceptance Hill Climbing (LAHC) search method with a window-based approach, SYCOS can automatically discover correlations at multiple temporal scales without requiring user inputs to specify the time scales or window sizes. 
	\item  Based on mutual information properties, we propose novel theories to identify noise in the data and estimate MI bounds, enabling efficient pruning of non-interesting time intervals from the search, thus significantly reducing the search space and improving the search speed. 
	\item  SYCOS is designed with an optimization engine to reuse the MI computation across a large number of windows, thus minimizing the computation redundancy and improving the speed. Moreover, SYCOS is scalable since it is designed in an efficient bottom-up fashion, making the method memory efficient and suitable for big datasets. 
	\item  Finally, we perform a comprehensive experimental evaluation using synthetic and real-world datasets from the energy and smart city domains, which shows that SYCOS is able to find important correlations among time series with high accuracy and is up to an order of magnitude faster than state-of-the-art techniques.
\end{itemize}




==> topdown.tex <==
\subsection{SYCOS$_{\text{TD}}$: Top-Down SYCOS}\label{sec:topdown}
In contrast to SYCOS$_{\text{BU}}$, the top-down method SYCOS$_{\text{TD}}$ addresses the SYCOS problem using a breath first search strategy: it starts with large-size windows, and reduces the window's size as the search progresses. Intuitively, SYCOS$_{\text{TD}}$ assumes that correlations exist in large-size windows, and thus is more efficient to start with large windows. Below, we discuss this approach in details.
 
\subsubsection{Multi-layer hierarchical top-down search}
SYCOS$_{\text{TD}}$ employs a multi-layer hierarchical top-down search in which the search space is divided into multiple layers, each corresponds to a specific window size. The top layer has the largest, and the lowest layer has the smallest window size. %In this tree-based structure, different layers have different window sizes, with the top layer (\textit{root}) corresponds to the largest, and the lowest layer (\textit{leaf}) corresponds to the smallest window size.
Furthermore, windows belong to the same layer share the same size. To keep track the size of windows among different layers, we use the concept of \textit{temporal scale}.

\textit{Definition 6.1} (\textit{Temporal scale}) 
A \textit{temporal scale} represents the size of windows belonging to the same layer in a multi-layer hierarchical search space. 

%SYCOS$_{\text{TD}}$ is a hierarchical search composed of multiple layers, each corresponding to a certain window size. Different layers in the hierarchy have different window sizes. Initially, the search starts at the top layer (root), and traverse to the lower layers until it reaches the lowest (leaf) layer of the tree. We describe each step below. 

%In a multi-layer hierarchical search tree, the upper layers have coarse temporal scales (corresponding to large windows), while lower layers have finer scales and smaller windows. For example, if the temporal scale of the top layer is \textit{year}, then the scales of lower layers can be \textit{month}, \textit{week},  \textit{day}, etc.  
%As windows of the same layer have equal size, they share the same temporal scale. For instance, if a layer has \textit{one month} as its temporal scale, then all windows belonging to this layer have the size equals to the data size measured in one month.

%The top layer corresponds to the largest window size, while the lowest layer corresponds to the smallest window size.  

Fig. \ref{fig:topdownsearchtree} depicts the multi-layer hierarchical search space, with the top layer L$_1$ has the largest temporal scale, and the bottom layer L$_n$ has the smallest temporal scale. 

To start the correlation search, initially, SYCOS$_{\text{TD}}$ begins at the top layer L$_1$ and search for correlated time series in the windows of size $s_{\max}$. To check whether a window $w$ contains correlated time series, the MI value of $w$, i.e., $I_{w}$, is computed and compared against the correlation threshold $\sigma$. If $I_{w} \ge \sigma$, the series in $w$ are correlated and thus $w$ is inserted into the result set $S$. Whereas if $I_{w} < \sigma$, the series of $w$ is not correlated, and $w$ will be passed to the lower layer L$_2$. SYCOS$_{\text{TD}}$ repeats this evaluation for every window of L$_1$. Once it completes, it traverses to the next layer L$_2$ and repeats the search with windows belong to L$_2$. SYCOS$_{\text{TD}}$ stops when it reaches the lowest layer L$_n$ which has windows of size $s_{\min}$. %, and finishes the search at this layer.

%To find well correlated windows, initially, the search starts at L$_1$ with the window size $s_{\max}$. At the beginning of the time series in L$_1$, the first window $w_1=[t_{s_1},t_{e_1}]$ is formed. To check whether $w_1$ is well correlated, the MI value of $w_1$,  i.e., $I_{w_1}$, is computed and compared against the correlation threshold $\sigma$. If $I_{w_1} \ge \sigma$, then $w_1$ is well correlated, and thus, is included in the result set $S$. Whereas if $I_{w_1} < \sigma$, then $w_1$ is not well correlated, and the data in $w_1$ will be passed to the lower layer L$_1$ where the search will start again on that data partition with smaller window size. %For windows that are not well correlated (MI values are less than $\sigma$). %  windows of this size are slided along the time series to identify those that are well correlated (by comparing to the predefined correlation threshold). At the same time, windows that are not correlated will be collected, and the data of these windows will be passed to lower layers, where the search will continue on uncorrelated data using smaller size windows. By using this multi-layer approach, correlations at multiple scales can be uncovered, and the computation cost can be minimized since lower layers only work on uncorrelated data filtered through the upper layers. 

\readdef{data/data.csv}\namedata
\readarray\namedata\timeseries[-,\ncols]
 \begin{figure}[!t]
	\centering
	%\begin{minipage}{0.42\linewidth}
	\begin{tikzpicture}%[yscale=0.5]
	\begin{axis}[axis line style={draw=none},
	tick style={draw=none},
	ymin = -20, ymax = 30,
	xmin = -40, xmax = 300,
	xticklabels={,,},
	yticklabels={,,}
	]
	\addplot [mark=none, blue] table [x=x, y=y1, col sep=comma] {data/data.csv};
	\addplot [mark=none, red] table [x=x, y=y2, col sep=comma] {data/data.csv};
	
	\node[black] (l1) at (axis cs: -30,-1) {\small L$_{1}$};
	
	\drawretangle {Apricot}{0}{-2}{90}{2}{\timeseries[2,3]}{\timeseries[81,3]}{\timeseries[2,2]}{\timeseries[81,2]};
	\drawretangle {Aquamarine}{30}{-3}{90}{2}{\timeseries[32,3]}{\timeseries[111,3]}{\timeseries[32,2]}{\timeseries[111,2]};
	\drawretangle {LimeGreen}{60}{-4}{90}{2}{\timeseries[62,3]}{\timeseries[141,3]}{\timeseries[62,2]}{\timeseries[141,2]};
	\drawretangle {Aquamarine}{90}{-5}{90}{2}{\timeseries[62,3]}{\timeseries[141,3]}{\timeseries[62,2]}{\timeseries[141,2]};
	\drawretangle {Red}{120}{-6}{90}{2}{\timeseries[92,3]}{\timeseries[171,3]}{\timeseries[92,2]}{\timeseries[171,2]};
	\drawretangle {Yellow}{210}{-2}{90}{2}{\timeseries[172,3]}{\timeseries[251,3]}{\timeseries[172,2]}{\timeseries[251,2]};
	
	\drawlabel {0}{-2}{90}{2}{1};
	\drawlabel {30}{-3}{90}{2}{2};
	\drawlabel {60}{-4}{90}{2}{3};
	\drawlabel {90}{-5}{90}{2}{4};
	\drawlabel {120}{-6}{90}{2}{5};
	\drawlabel {210}{-2}{90}{2}{6};
	
	
	\node[black] (l2) at (axis cs: -30,-8) {\small L$_{2}$};
	
	
	\draw [black ,thin,dashed] (axis cs: -0.99 , -2) -- (axis cs: -0.99,-10);
	\draw [black ,thin,dashed] (axis cs: 120 , -5) -- (axis cs: 120,-10);
	
	\drawretangleonly {Apricot}{0}{-9}{40}{2};
	\drawretangleonly {Red}{30}{-9.5}{40}{2};
	
	
	
	\node[black] (ln) at (axis cs: -30,-18) {\small L$_{n}$};
	\path (l2) -- (ln) node [black, font=\small, midway, sloped] {$\dots$};
	
	\drawretangleonly {Apricot}{0}{-19}{30}{2};
	\end{axis}
	\end{tikzpicture}%
	\caption{Multi-layer hierarchical search tree} 
	%\vspace{-0.1in}
	\label{fig:topdownsearchtree}
	%\end{minipage}	
\end{figure}	

%At each layer, same-size windows are slided along the time series to identify those that are well correlated (by comparing to the predefined correlation threshold). When moving from one window to another, two consecutive windows are shifted a $\delta$-step. For windows that are not well correlated, they will be collected to pass to lower layers. Figure depicts the top-down search process.

%Initially, the top-down search starts with the largest window size. At each layer, equal-sized windows are slided along the time series to identify those that are well-correlated with respect to the predefined correlation threshold. 
%Initially, the search starts with the coarsest granularity, i.e., the largest window size. %, and try to search for temporal correlations in that size. 
%Data partitions that do not contain interesting correlations in that layer will be passed to lower layers, to be searched with finer granularity. 

%Moreover, the computation within the same layer is performed incrementally, thus eliminating redundant computation.
%\subsubsection{Top-down Filtering with Adaptive Window Size}\label{sec:topdown}
%\textit{Definition 1.} Given two time series $X=\{x_{t}\}^{N}_{t=1}$ and $Y=\{y_{t}\}^{N}_{t=1}$, a \textit{time window $w_{X,Y}$} of $(X,Y)$ is a sequence of timestamped data points $(x_t,y_t)$ %$\in \{(x_t,y_t)\}^{N}_{t=1}$, collected over a continuous time interval and sorted in chronological order.

%We allow user to define the \textit{maximum} ($g_{max}$) and the \textit{minimum} ($g_{min}$) granularity s/he wants to operate on the data, as well as the \textit{sliding step} by which the window will be shifted. Starting with the largest granularity, data are partitioned into windows of the same size. 

%Using \textit{KSG} estimator, the MI value is computed for each window and is compared against the threshold $\sigma$. Windows that have significant correlations (i.e., $\ge \sigma$) are selected. 

%The search stops when it reaches the lowest layer in the tree that has the \textit{minimum} temporal scale (minimum window size $s_{\min}$). 
%With this layered top-down approach, user has the flexibility to search for dependencies at different time scales. To test if the variables of interest are overall correlated, user can set the \textit{maximum} scale covering the entire time series, while iteratively reducing the temporal scale in lower layers helps uncover correlations in different time durations. For example, when searching for correlations between taxi and weather data, user can start with \textit{year} scale, then reduce to \textit{month}, \textit{week}, \textit{day}, and \textit{hour}. 
\subsubsection{Filtering using sliding window} \label{sec:slidingfilter}
At each layer in the hierarchical search space, SYCOS$_{\text{TD}}$ perform the search by sliding a window of a specific size along the time series, and windows whose MI greater than the threshold $\sigma$ are selected, while uncorrelated windows (called \textit{left-out} data) are collected and passed to the lower layer for the next scan. Two consecutive windows can be either disjoint or overlapping depending on whether significant correlation exists in one of them. We illustrate this sliding movement in Fig. \ref{fig:topdownsearchtree}.  

%At each layer in the hierarchical search space, SYCOS$_{\text{TD}}$ will return a set of well correlated windows that have MI greater than the threshold $\sigma$, and a set of uncorrelated windows. These uncorrelated windows (called \textit{left-out} data) are collected and passed to the lower layer for the next scan. In this section, we describe the search procedure to find correlated windows at each individual layer. 
%For example, at L$_0$, it scans the entire time series, while at L$_1$, the \textit{left-out} data partitions passing from L$_0$ can be used. 
\textit{Definition 6.2} ($\delta$-step) A $\delta$-step is a sliding step by which two consecutive windows in the same layer are shifted from one to the other. %from its current time window to the next time window. % in the direction towards the future.  

The $\delta$-step represents how far the current window should be shifted to form the next window. %For example, if the $\delta$-step is set to one hour, then the current window is shifted by one hour when it moves to the next window. 

As an example, assume that $w_1$, $w_2$, $w_3$ and $w_4$ in Fig. \ref{fig:topdownsearchtree} are not well correlated, and thus, the data partition from t$_{s_1}$ to t$_{s_5}$ is passed to L$_2$ for the next scan.

%%\begin{figure}[!h]
%%	\centering
%%	\includegraphics[width=0.4\textwidth]{Figures/slidingwindow}
%%	\caption{Filtering using sliding window}
%%	\label{fig:slidingwindow}
%%\end{figure} 

%Consider the pair of variables $(X,Y)$, each window $w_{i}$ is identified by the start index $s_{i}$ and the end index $e_{i}$ (indicating the first and the last data point of $w_{i}$). Since each data point is associated with a timestamp, the start and end index also indicate the window's start and end time. We use the data structures \textit{left-out} list and \textit{windows} list to store the \textit{left-out} data and the \textit{selected} windows. Let $\sigma_{i}$ be the computed MI value of $w_{i}$.

At L$_1$ in Fig. \ref{fig:topdownsearchtree}, the search starts from the left edge of the data  partition, and forms the first window $w_{1}=[t_{s_{1}},t_{e_{1}}]$. Assuming that $I_{w_1}<\sigma$, then $w_{1}$ does not satisfy the correlation threshold, and its indices $[t_{s_{1}},t_{e_{1}}]$ are inserted into a \textit{left-out} list containing uncorrelated windows. 
Next, the search shifts $w_1$ by a $\delta$-step to the right, creating the next window $w_2=[t_{s_2},t_{e_2}]$ and computing $I_{w_2}$.
As illustrated in Fig. \ref{fig:topdownsearchtree}, we also assume $I_{w_2} < \sigma$, and thus, $w_2$ is inserted into the \textit{left-out} list. Since $w_1$ and $w_2$ are consecutive, the indices in \textit{left-out} list are modified to $[t_{s_{1}},t_{e_{2}}]$, indicating that a data partition from $t_{s_{1}}$ to $t_{e_{2}}$ contains uncorrelated data. Similarly, $w_3$ and $w_4$ do not satisfy the threshold, and the \textit{left-out} list is changed to $[t_{s_{1}},t_{e_{4}}]$. At $w_5$, we have $I_{w_5} \ge \sigma$, and thus, $w_5$ contains correlated data and is inserted into the result set $S$. At the same time, the \textit{left-out} list is updated to $[t_{s_1},t_{s_5}]$, indicating that only data from $t_{s_1}$ to $t_{s_5}$ are uncorrelated and will be passed to the next layer. The search moves on to the next window $w_6=[t_{s_6},t_{e_6}]$ where $t_{s_6}$ is right after $t_{e_5}$ of $w_5$. The procedure is repeated until the end of the current data partition.
Algorithm \ref{alg:topdownsearch} provides the outline of this multi-layer hierarchical top-down search for SYCOS.
%Fig. \ref{fig:slidingwindow1} illustrates the results after the first scan. A set of non-overlapping windows which hold significant correlations is stored in the \textit{windows} list, and a set of disjoint data partitions containing left out data is stored in the \textit{left-out} list. These left out data partitions will become the inputs for the next scan with finer granularity.
%%\begin{figure}[!t]
%%	\centering
%%	\includegraphics[width=0.4\textwidth]{Figures/slidingwindow1}
%%	\caption{Time series after the first scan}
%%	\label{fig:slidingwindow1}
%%\end{figure}

%\begin{figure*}[!t]
%\centering
%\subfigure[Adaptive sliding %window]{\includegraphics[scale=0.85]{Figures/slidingwindow}\label{fig:slidingwindow}} \quad
%\subfigure[Time series after one %scan]{\includegraphics[scale=0.85]{Figures/slidingwindow1}\label{fig:slidingwindow1}}
%\caption{Mutual information search algorithm}
%\end{figure*}

%Algorithm \ref{alg:topdownsearch} presents pseudo-code implementation of top-down search using sliding window. In step $1$, the search start searching the MI along the data series with current granularity $curgra$. The results of this scan will be the set of $satisfiedWindows$ and $unSatisfiedWindows$. If number of unsatisfied windows $wCount$ are still greater than $0$ and the granularity is not the minimum, the search repeatedly $searchMI$ process in \textit{step 2} with smaller granularity until either no unsatisfied windows is left or the granularity reaches the minimum.

%\textbf{Correct this algorithm}

%\begin{algorithm}
%\caption{Dynamic Sliding Window Top-down Search}
%\label{alg:topdownsearch}
%\begin{algorithmic}
%\STATE \textbf{Inputs:} $<x,y>$: time series variables
%\STATE \textbf{Parameters:} $wSize$: window size, $curgra$: current granularity
%\WHILE{$curgra > 0$}
%\STATE wCount = searchMI(data, curgra, satisfiedWindows, unSatisfiedWindows);
%\IF{$wCount > 0$}
%\STATE pregra=curgra
%\STATE curgra = curgra - 1
%\STATE wCount = searchMI(data, curgra, satisfiedWindows, unSatisfiedWindows);
%\ENDIF
%\ENDWHILE
%\end{algorithmic}
%\end{algorithm}
%\vspace{-0.25cm}

\begin{algorithm}
	\caption{Top-Down Approach for SYCOS (SYCOS$_{\text{TD}}$)}
	\footnotesize
	\begin{algorithmic}[1]
		\Statex{{\bf Input:}} $\{X_T,Y_T\}$: \text{pair of time series} 
		\Statex{{\bf Params:} $\sigma$: \text{correlation threshold,}} 
		\Statex{\hspace{1.07cm}$\delta$: \text{sliding step,}} 
		\Statex{\hspace{1.07cm}$s_{\max}$: \text{maximum window size,}} 
		\Statex{\hspace{1.07cm}$s_{\min}$: \text{minimum window size}} 
		\Statex{{\bf Output:} $S$: \text{set of non-overlapping windows with MI $\ge \sigma$}}
		
		\State{\textit{Initialize:} $s_w \gets s_{\max}$, $\textit{leftOutList} \gets \{X_T,Y_T\}$}
		\While{$s_{w} \ge s_{\min}$}
		\While{notEmpty({$\textit{leftOutList}$})}
		\State {$\textit{leftOut}$ $\gets$ {$\textit{leftOutList.next}$}} \Comment{gets the next element in \textit{left-out} list}
		\State \text{$w$ $\gets$ getNextWindow({$\textit{leftOut}$}$,s_{w})$} \Comment{gets the next window from the current \textit{left-out} partition with size $s_w$}
		\While{\text{$\textit{w.endIndex}$ $\le$ $\textit{leftOut.endIndex}$}} 
		\State	 \text{$I_w$ $\gets$ computeMI($w$)} \Comment{compute MI value}
		\If{\text{$I_w \ge \sigma$}}
		\State \text{$\mathit{S}$.insert($w$)} 
		\State {$w$ $\gets$ getNextWindow($\textit{leftOut},s_w)$}
		\Else
		\State \text{$w$ $\gets$ shiftWindow($\textit{leftOut},s_w,\delta)$} 
		\State \text{update($\textit{LeftOutList}$)}
		\EndIf
		\EndWhile
		\EndWhile
		\State $s_w  \gets \text{reduce}(s_w)$ \Comment{reduce the temporal scale in lower layer}
		\EndWhile
		\State \text{\textbf{return} $\mathit{S}$}
		%\EndFunction
		%\Statex{\bf end function}
	\end{algorithmic}
	\label{alg:topdownsearch}
\end{algorithm}



==> topdown_bk.tex <==
\section{SYCOS$_{\text{TD}}$: Top-Down SYCOS}\label{sec:topdown}
In contrast to SYCOS$_{\text{BU}}$, the top-down method SYCOS$_{\text{TD}}$ addresses the SYCOS problem using a breath first search strategy: it starts with large-size windows, and reduces the window's size as the search progresses. Intuitively, SYCOS$_{\text{TD}}$ assumes that correlations exist in large-size windows, and thus is more efficient to start with large windows. Below, we discuss this approach in details.
 
\subsection{Multi-layer hierarchical top-down search}
SYCOS$_{\text{TD}}$ employs a multi-layer hierarchical top-down search in which the search space is divided into multiple layers, each corresponds to a specific window size. The top layer has the largest, and the lowest layer has the smallest window size. %In this tree-based structure, different layers have different window sizes, with the top layer (\textit{root}) corresponds to the largest, and the lowest layer (\textit{leaf}) corresponds to the smallest window size.
Furthermore, windows belong to the same layer share the same size. To keep track the size of windows among different layers, we use the concept of \textit{temporal scale}.

\textit{Definition 6.1} (\textit{Temporal scale}) 
A \textit{temporal scale} represents the size of windows belonging to the same layer in a multi-layer hierarchical search space. 

%SYCOS$_{\text{TD}}$ is a hierarchical search composed of multiple layers, each corresponding to a certain window size. Different layers in the hierarchy have different window sizes. Initially, the search starts at the top layer (root), and traverse to the lower layers until it reaches the lowest (leaf) layer of the tree. We describe each step below. 

%In a multi-layer hierarchical search tree, the upper layers have coarse temporal scales (corresponding to large windows), while lower layers have finer scales and smaller windows. For example, if the temporal scale of the top layer is \textit{year}, then the scales of lower layers can be \textit{month}, \textit{week},  \textit{day}, etc.  
%As windows of the same layer have equal size, they share the same temporal scale. For instance, if a layer has \textit{one month} as its temporal scale, then all windows belonging to this layer have the size equals to the data size measured in one month.

%The top layer corresponds to the largest window size, while the lowest layer corresponds to the smallest window size.  

Fig. \ref{fig:topdownsearchtree} depicts the multi-layer hierarchical search space, with the top layer L$_1$ has the largest temporal scale, and the bottom layer L$_n$ has the smallest temporal scale. 

To start the correlation search, initially, SYCOS$_{\text{TD}}$ begins at the top layer L$_1$ and search for correlated time series in the windows of size $s_{\max}$. To check whether a window $w$ contains correlated time series, the MI value of $w$, i.e., $I_{w}$, is computed and compared against the correlation threshold $\sigma$. If $I_{w} \ge \sigma$, the series in $w$ are correlated and thus $w$ is inserted into the result set $S$. Whereas if $I_{w} < \sigma$, the series of $w$ is not correlated, and $w$ will be passed to the lower layer L$_2$. SYCOS$_{\text{TD}}$ repeats this evaluation for every window of L$_1$. Once it completes, it traverses to the next layer L$_2$ and repeats the search with windows belong to L$_2$. SYCOS$_{\text{TD}}$ stops when it reaches the lowest layer L$_n$ which has windows of size $s_{\min}$. %, and finishes the search at this layer.

%To find well correlated windows, initially, the search starts at L$_1$ with the window size $s_{\max}$. At the beginning of the time series in L$_1$, the first window $w_1=[t_{s_1},t_{e_1}]$ is formed. To check whether $w_1$ is well correlated, the MI value of $w_1$,  i.e., $I_{w_1}$, is computed and compared against the correlation threshold $\sigma$. If $I_{w_1} \ge \sigma$, then $w_1$ is well correlated, and thus, is included in the result set $S$. Whereas if $I_{w_1} < \sigma$, then $w_1$ is not well correlated, and the data in $w_1$ will be passed to the lower layer L$_1$ where the search will start again on that data partition with smaller window size. %For windows that are not well correlated (MI values are less than $\sigma$). %  windows of this size are slided along the time series to identify those that are well correlated (by comparing to the predefined correlation threshold). At the same time, windows that are not correlated will be collected, and the data of these windows will be passed to lower layers, where the search will continue on uncorrelated data using smaller size windows. By using this multi-layer approach, correlations at multiple scales can be uncovered, and the computation cost can be minimized since lower layers only work on uncorrelated data filtered through the upper layers. 

\readdef{data/data.csv}\namedata
\readarray\namedata\timeseries[-,\ncols]
 \begin{figure}[!t]
	\centering
	%\begin{minipage}{0.42\linewidth}
	\begin{tikzpicture}%[yscale=0.5]
	\begin{axis}[axis line style={draw=none},
	tick style={draw=none},
	ymin = -20, ymax = 30,
	xmin = -40, xmax = 300,
	xticklabels={,,},
	yticklabels={,,}
	]
	\addplot [mark=none, blue] table [x=x, y=y1, col sep=comma] {data/data.csv};
	\addplot [mark=none, red] table [x=x, y=y2, col sep=comma] {data/data.csv};
	
	\node[black] (l1) at (axis cs: -30,-1) {\small L$_{1}$};
	
	\drawretangle {Apricot}{0}{-2}{90}{2}{\timeseries[2,3]}{\timeseries[81,3]}{\timeseries[2,2]}{\timeseries[81,2]};
	\drawretangle {Aquamarine}{30}{-3}{90}{2}{\timeseries[32,3]}{\timeseries[111,3]}{\timeseries[32,2]}{\timeseries[111,2]};
	\drawretangle {LimeGreen}{60}{-4}{90}{2}{\timeseries[62,3]}{\timeseries[141,3]}{\timeseries[62,2]}{\timeseries[141,2]};
	\drawretangle {Aquamarine}{90}{-5}{90}{2}{\timeseries[62,3]}{\timeseries[141,3]}{\timeseries[62,2]}{\timeseries[141,2]};
	\drawretangle {Red}{120}{-6}{90}{2}{\timeseries[92,3]}{\timeseries[171,3]}{\timeseries[92,2]}{\timeseries[171,2]};
	\drawretangle {Yellow}{210}{-2}{90}{2}{\timeseries[172,3]}{\timeseries[251,3]}{\timeseries[172,2]}{\timeseries[251,2]};
	
	\drawlabel {0}{-2}{90}{2}{1};
	\drawlabel {30}{-3}{90}{2}{2};
	\drawlabel {60}{-4}{90}{2}{3};
	\drawlabel {90}{-5}{90}{2}{4};
	\drawlabel {120}{-6}{90}{2}{5};
	\drawlabel {210}{-2}{90}{2}{6};
	
	
	\node[black] (l2) at (axis cs: -30,-8) {\small L$_{2}$};
	
	
	\draw [black ,thin,dashed] (axis cs: -0.99 , -2) -- (axis cs: -0.99,-10);
	\draw [black ,thin,dashed] (axis cs: 120 , -5) -- (axis cs: 120,-10);
	
	\drawretangleonly {Apricot}{0}{-9}{40}{2};
	\drawretangleonly {Red}{30}{-9.5}{40}{2};
	
	
	
	\node[black] (ln) at (axis cs: -30,-18) {\small L$_{n}$};
	\path (l2) -- (ln) node [black, font=\small, midway, sloped] {$\dots$};
	
	\drawretangleonly {Apricot}{0}{-19}{30}{2};
	\end{axis}
	\end{tikzpicture}%
	\caption{Multi-layer hierarchical search tree} 
	%\vspace{-0.1in}
	\label{fig:topdownsearchtree}
	%\end{minipage}	
\end{figure}	

%At each layer, same-size windows are slided along the time series to identify those that are well correlated (by comparing to the predefined correlation threshold). When moving from one window to another, two consecutive windows are shifted a $\delta$-step. For windows that are not well correlated, they will be collected to pass to lower layers. Figure depicts the top-down search process.

%Initially, the top-down search starts with the largest window size. At each layer, equal-sized windows are slided along the time series to identify those that are well-correlated with respect to the predefined correlation threshold. 
%Initially, the search starts with the coarsest granularity, i.e., the largest window size. %, and try to search for temporal correlations in that size. 
%Data partitions that do not contain interesting correlations in that layer will be passed to lower layers, to be searched with finer granularity. 

%Moreover, the computation within the same layer is performed incrementally, thus eliminating redundant computation.
%\subsubsection{Top-down Filtering with Adaptive Window Size}\label{sec:topdown}
%\textit{Definition 1.} Given two time series $X=\{x_{t}\}^{N}_{t=1}$ and $Y=\{y_{t}\}^{N}_{t=1}$, a \textit{time window $w_{X,Y}$} of $(X,Y)$ is a sequence of timestamped data points $(x_t,y_t)$ %$\in \{(x_t,y_t)\}^{N}_{t=1}$, collected over a continuous time interval and sorted in chronological order.

%We allow user to define the \textit{maximum} ($g_{max}$) and the \textit{minimum} ($g_{min}$) granularity s/he wants to operate on the data, as well as the \textit{sliding step} by which the window will be shifted. Starting with the largest granularity, data are partitioned into windows of the same size. 

%Using \textit{KSG} estimator, the MI value is computed for each window and is compared against the threshold $\sigma$. Windows that have significant correlations (i.e., $\ge \sigma$) are selected. 

%The search stops when it reaches the lowest layer in the tree that has the \textit{minimum} temporal scale (minimum window size $s_{\min}$). 
%With this layered top-down approach, user has the flexibility to search for dependencies at different time scales. To test if the variables of interest are overall correlated, user can set the \textit{maximum} scale covering the entire time series, while iteratively reducing the temporal scale in lower layers helps uncover correlations in different time durations. For example, when searching for correlations between taxi and weather data, user can start with \textit{year} scale, then reduce to \textit{month}, \textit{week}, \textit{day}, and \textit{hour}. 
\subsection{Filtering using sliding window} \label{sec:slidingfilter}
At each layer in the hierarchical search space, SYCOS$_{\text{TD}}$ perform the search by sliding a window of a specific size along the time series, and windows whose MI greater than the threshold $\sigma$ are selected, while uncorrelated windows (called \textit{left-out} data) are collected and passed to the lower layer for the next scan. Two consecutive windows can be either disjoint or overlapping depending on whether significant correlation exists in one of them. We illustrate this sliding movement in Fig. \ref{fig:topdownsearchtree}.  

%At each layer in the hierarchical search space, SYCOS$_{\text{TD}}$ will return a set of well correlated windows that have MI greater than the threshold $\sigma$, and a set of uncorrelated windows. These uncorrelated windows (called \textit{left-out} data) are collected and passed to the lower layer for the next scan. In this section, we describe the search procedure to find correlated windows at each individual layer. 
%For example, at L$_0$, it scans the entire time series, while at L$_1$, the \textit{left-out} data partitions passing from L$_0$ can be used. 
\textit{Definition 6.2} ($\delta$-step) A $\delta$-step is a sliding step by which two consecutive windows in the same layer are shifted from one to the other. %from its current time window to the next time window. % in the direction towards the future.  

The $\delta$-step represents how far the current window should be shifted to form the next window. %For example, if the $\delta$-step is set to one hour, then the current window is shifted by one hour when it moves to the next window. 

As an example, assume that $w_1$, $w_2$, $w_3$ and $w_4$ in Fig. \ref{fig:topdownsearchtree} are not well correlated, and thus, the data partition from t$_{s_1}$ to t$_{s_5}$ is passed to L$_2$ for the next scan.



%%\begin{figure}[!h]
%%	\centering
%%	\includegraphics[width=0.4\textwidth]{Figures/slidingwindow}
%%	\caption{Filtering using sliding window}
%%	\label{fig:slidingwindow}
%%\end{figure} 

%Consider the pair of variables $(X,Y)$, each window $w_{i}$ is identified by the start index $s_{i}$ and the end index $e_{i}$ (indicating the first and the last data point of $w_{i}$). Since each data point is associated with a timestamp, the start and end index also indicate the window's start and end time. We use the data structures \textit{left-out} list and \textit{windows} list to store the \textit{left-out} data and the \textit{selected} windows. Let $\sigma_{i}$ be the computed MI value of $w_{i}$.

At L$_1$ in Fig. \ref{fig:topdownsearchtree}, the search starts from the left edge of the data  partition, and forms the first window $w_{1}=[t_{s_{1}},t_{e_{1}}]$. Assuming that $I_{w_1}<\sigma$, then $w_{1}$ does not satisfy the correlation threshold, and its indices $[t_{s_{1}},t_{e_{1}}]$ are inserted into a \textit{left-out} list containing uncorrelated windows. 
Next, the search shifts $w_1$ by a $\delta$-step to the right, creating the next window $w_2=[t_{s_2},t_{e_2}]$ and computing $I_{w_2}$.
As illustrated in Fig. \ref{fig:topdownsearchtree}, we also assume $I_{w_2} < \sigma$, and thus, $w_2$ is inserted into the \textit{left-out} list. Since $w_1$ and $w_2$ are consecutive, the indices in \textit{left-out} list are modified to $[t_{s_{1}},t_{e_{2}}]$, indicating that a data partition from $t_{s_{1}}$ to $t_{e_{2}}$ contains uncorrelated data. Similarly, $w_3$ and $w_4$ do not satisfy the threshold, and the \textit{left-out} list is changed to $[t_{s_{1}},t_{e_{4}}]$. At $w_5$, we have $I_{w_5} \ge \sigma$, and thus, $w_5$ contains correlated data and is inserted into the result set $S$. At the same time, the \textit{left-out} list is updated to $[t_{s_1},t_{s_5}]$, indicating that only data from $t_{s_1}$ to $t_{s_5}$ are uncorrelated and will be passed to the next layer. The search moves on to the next window $w_6=[t_{s_6},t_{e_6}]$ where $t_{s_6}$ is right after $t_{e_5}$ of $w_5$. The procedure is repeated until the end of the current data partition.
Algorithm \ref{alg:topdownsearch} provides the outline of this multi-layer hierarchical top-down search for SYCOS.
%Fig. \ref{fig:slidingwindow1} illustrates the results after the first scan. A set of non-overlapping windows which hold significant correlations is stored in the \textit{windows} list, and a set of disjoint data partitions containing left out data is stored in the \textit{left-out} list. These left out data partitions will become the inputs for the next scan with finer granularity.
%%\begin{figure}[!t]
%%	\centering
%%	\includegraphics[width=0.4\textwidth]{Figures/slidingwindow1}
%%	\caption{Time series after the first scan}
%%	\label{fig:slidingwindow1}
%%\end{figure}

%\begin{figure*}[!t]
%\centering
%\subfigure[Adaptive sliding %window]{\includegraphics[scale=0.85]{Figures/slidingwindow}\label{fig:slidingwindow}} \quad
%\subfigure[Time series after one %scan]{\includegraphics[scale=0.85]{Figures/slidingwindow1}\label{fig:slidingwindow1}}
%\caption{Mutual information search algorithm}
%\end{figure*}

%Algorithm \ref{alg:topdownsearch} presents pseudo-code implementation of top-down search using sliding window. In step $1$, the search start searching the MI along the data series with current granularity $curgra$. The results of this scan will be the set of $satisfiedWindows$ and $unSatisfiedWindows$. If number of unsatisfied windows $wCount$ are still greater than $0$ and the granularity is not the minimum, the search repeatedly $searchMI$ process in \textit{step 2} with smaller granularity until either no unsatisfied windows is left or the granularity reaches the minimum.

%\textbf{Correct this algorithm}

%\begin{algorithm}
%\caption{Dynamic Sliding Window Top-down Search}
%\label{alg:topdownsearch}
%\begin{algorithmic}
%\STATE \textbf{Inputs:} $<x,y>$: time series variables
%\STATE \textbf{Parameters:} $wSize$: window size, $curgra$: current granularity
%\WHILE{$curgra > 0$}
%\STATE wCount = searchMI(data, curgra, satisfiedWindows, unSatisfiedWindows);
%\IF{$wCount > 0$}
%\STATE pregra=curgra
%\STATE curgra = curgra - 1
%\STATE wCount = searchMI(data, curgra, satisfiedWindows, unSatisfiedWindows);
%\ENDIF
%\ENDWHILE
%\end{algorithmic}
%\end{algorithm}
%\vspace{-0.25cm}

\begin{algorithm}
	\caption{Top-Down Approach for SYCOS (SYCOS$_{\text{TD}}$)}
	\footnotesize
	\begin{algorithmic}[1]
		\Statex{{\bf Input:}} $\{X_T,Y_T\}$: \text{pair of time series} 
		\Statex{{\bf Params:} $\sigma$: \text{correlation threshold,}} 
		\Statex{\hspace{1.07cm}$\delta$: \text{sliding step,}} 
		\Statex{\hspace{1.07cm}$s_{\max}$: \text{maximum window size,}} 
		\Statex{\hspace{1.07cm}$s_{\min}$: \text{minimum window size}} 
		\Statex{{\bf Output:} $S$: \text{set of non-overlapping windows with MI $\ge \sigma$}}
		
		\State{\textit{Initialize:} $s_w \gets s_{\max}$, $\textit{leftOutList} \gets \{X_T,Y_T\}$}
		\While{$s_{w} \ge s_{\min}$}
		\While{notEmpty({$\textit{leftOutList}$})}
		\State {$\textit{leftOut}$ $\gets$ {$\textit{leftOutList.next}$}} \Comment{gets the next element in \textit{left-out} list}
		\State \text{$w$ $\gets$ getNextWindow({$\textit{leftOut}$}$,s_{w})$} \Comment{gets the next window from the current \textit{left-out} partition with size $s_w$}
		\While{\text{$\textit{w.endIndex}$ $\le$ $\textit{leftOut.endIndex}$}} 
		\State	 \text{$I_w$ $\gets$ computeMI($w$)} \Comment{compute MI value}
		\If{\text{$I_w \ge \sigma$}}
		\State \text{$\mathit{S}$.insert($w$)} 
		\State {$w$ $\gets$ getNextWindow($\textit{leftOut},s_w)$}
		\Else
		\State \text{$w$ $\gets$ shiftWindow($\textit{leftOut},s_w,\delta)$} 
		\State \text{update($\textit{LeftOutList}$)}
		\EndIf
		\EndWhile
		\EndWhile
		\State $s_w  \gets \text{reduce}(s_w)$ \Comment{reduce the temporal scale in lower layer}
		\EndWhile
		\State \text{\textbf{return} $\mathit{S}$}
		%\EndFunction
		%\Statex{\bf end function}
	\end{algorithmic}
	\label{alg:topdownsearch}
\end{algorithm}


